Design, Implementation, and Automation of a Risk Management Approach for Man-at-the-End Software Protection

The last years have seen an increase in Man-at-the-End (MATE) attacks against software applications, both in number and severity. However, software protection, which aims at mitigating MATE attacks, is dominated by fuzzy concepts and security-through-obscurity. This paper presents a rationale for adopting and standardizing the protection of software as a risk management process according to the NIST SP800-39 approach. We examine the relevant constructs, models, and methods needed for formalizing and automating the activities in this process in the context of MATE software protection. We highlight the open issues that the research community still has to address. We discuss the benefits that such an approach can bring to all stakeholders. In addition, we present a Proof of Concept (PoC) decision support system that instantiates many of the discussed construct, models, and methods and automates many activities in the risk analysis methodology for the protection of software. Despite being a prototype, the PoC's validation with industry experts indicated that several aspects of the proposed risk management process can already be formalized and automated with our existing toolbox and that it can actually assist decision-making in industrially relevant settings.

==> attack.tex <==
\begin{itemize}
    %\item useless intro
    %\item security requirements description (maybe move into intro/requirements chapter)
    \item brief description of attack paths/trees (refs to attack trees theory + other security applications)
    \item difficulties (i.e. why coarse attack steps = backward programming combinatorial explosion + no way to automatically model actual attack steps)
    \item general work-flow of attack finder + description
\end{itemize}

%This chapter presents the risk assessment method used by \esp to infer possible attacks against the application assets in the vanilla application, \ie the unprotected program. As detailed in Section~\ref{sec:esp:workflow:model}, \esp, prior to this phase, executes a preliminary analysis of the source code, enriching the \ekb with the description of the application structure, instancing the related meta-model classes described in Section~\ref{sec:model:app}. The risk assessment phase employs this information, in order to infer attacks tailored to the specific application examined. Each attack aims to breach a security requirement of an application asset; these are provided by the user, annotating the application source code as detailed in Section~\ref{sec:esp:impl:solDep}.

%The definition of security requirements stem from the \nist guide to risk management \cite{nistSP800-39}, which defines the \textit{confidentiality} and the \textit{integrity} of assets. In this thesis, two new additional requirements are introduced, in order to adapt to the application security scenario.

%\esp supports three security requirements for assets: \textit{confidentiality}, \textit{integrity}, \textit{execution correctness}. A confidential asset must not be understandable by an attacker: this is the case for example of an algorithm that must remain secret, in order to safeguard the software company IP, or of a data structure that holds personal information of the user, such as the credit card number in an e-commerce application. The integrity requirement specifies that an asset must not be modifiable by an attacker: for example, in the case of a soccer video-game, the variables holding the characteristics of the soccer players, or the match score, can be marked with the integrity requirement, in order to avoid an attacker to cheat. The execution correctness requirement is a stronger form of integrity for code: the latter must not be modified, but must also be called as expected by other functions. For example, an attacker that wants to remove a license check function, marked with this requirement, may modify the function in order to not perform the check, but can also avoid the function to be executed, removing any calls by other functions to the license check one.

%
%Weak confidentiality is a particular case of the previous requirements, breached when the attacker is able to get a datum value in every moment of the application execution. For example, e-banking websites typically employ a two-factor authentication: to access its account, and every time it executes a security-sensitive operation (\eg a money transfer to another bank account), the user must not only provide its credentials, but also a \otp, valid only to authorize a single operation. \glspl{otp} are typically generated either using a hardware dongle, or with a mobile application. In the second case, the \otp is generation is based on a pre-shared secret among the mobile application and the e-banking server, and on a factor that changes every time a new \otp is requested by the user: for example, a counter that is incremented every time a new \otp is generated. An attacker, which has already stolen the access credentials of a user, may be interested in being able to generate such passwords at will, hacking the \otp generator. Even in the most simple case, when the attacker wants to access the e-banking account, and then transfer all the money to its account, the attacker needs to obtain two \glspl{otp}: one to access
%
%Some data may be also tagged
%with the weak confidentiality property. This property is breached when the attacker
%is able to retrieve the datum at every moment of the application execution
%(thus for hard-coded data the weak confidentiality is the same as the normal
%confidentiality). This is mostly interesting for attacks that target the assets of a
%victim’s application (i.e., not the attacker’s copy) by means of a distributed approach
%aiming at continuously obtaining the data values. For instance, in case of
%an OTP (One-Time Password) generator1 that generates the next password by
%hashing the value of a fixed seed and a counter modified at each generation, the
%variable storing the counter can be marked with weak confidentiality. To predict
%the next passwords (not only the next one), it does not suffice that the attacker
%obtains once the value of victim’s counter, he has to obtain it just before every
%generation. Therefore, either he is able to access every time the victim’s application to read the counter value, or he has to obtain one counter, understand
%the counter update function, and reproduce it on his copy.
%

%\esp models attacks against such security requirements with \textit{attack paths}, which are sequences of simple tasks that an attacker may execute (\eg locating a variable in the binary, debugging a function at run-time), called \textit{attack steps}: this modelling approach has already been used by other works in literature for risk assessment of computer networks \cite{ekelhart,fenz}. Each attack step is associated with a set of postconditions, which model the result of a successful execution by the attacker of the simple task related to the step, and a set of preconditions, which must be fulfilled by the results of other steps preceding it in the path. Attack steps may contain also preconditions about the application structure: for example, an attack step modelling the debugging of a function, can be executed only if the analyzed asset is a code and not a variable.
%Attack steps are modeled as Horn clauses \cite{hornClauses} (see Section~\ref{sec:background:expSys:inf}), and are stored in the \ekb as rules written in the Prolog language.

%\esp, to infer the possible attack paths against the asset security requirements of the target application, relies on an external inference engine, where attack steps are modelled as logical rules. At the start of the risk assessment phase, \esp instructs the engine about the structure of the application, modelling each concept of the application meta-model (see Section~\ref{sec:model:app}) as an axiom, \ie a fact that engine knows to be true. Then, \esp queries the engine, for each asset security requirement, to prove that the attacker can breach it: to do this, the engine tries to find every possible chain of rules (\ie a sequence of attack steps forming an attack path), which can be ultimately proven with a subset of the aforementioned axioms about the application structure. The engine carries out this task using a backward programming algorithm (see Section~\ref{sec:background:expSys:inf}). Other works in literature \cite{ou,kagal} have already used a similar approach to assess risk for computer networks. To ease readability, in the remainder of this chapter attack steps and axioms are expressed with the mathematical proofs notation. 

%The attack steps are modelled with the following inference rules:
% \begin{equation*}
% \infer[id,]{C}{P}
% \end{equation*}
% Where:
% \begin{itemize}
% 	\item $id$ is the name that identifies the attack step;
% 	\item $P$ is a set of facts, called \emph{premises}: if these facts are verified, the attack step can be executed by the attacker;
% 	\item $C$ is a set of facts, called \emph{conclusions}: these facts will be verified if the attack step can be carried out by the attacker.
% \end{itemize}

% The user can influence the time needed to infer the possible attack steps with two parameters. First, he or she can set a hard time limit (expressed in seconds). Also, he or she can decide a limit for the backward programming algorithm, in term of number of traversed relationships among application parts (\eg the maximum distance among application parts in the call graph), when the algorithm is searching for an attack step that, with its conclusions, can satisfy a premise of another attack step.

% Finally, the attack paths are saved in the \esp \ekb, structured using the related classes described in the meta-model (Section~\ref{sec:model:att}). The attacks are then used in the risk mitigation phase of \esp: during the latter, the protections best suitable to protect the application assets, against the attack paths previously found by the inference engine.

% This chapter is a reworked version of the publication ``Towards Automatic Risk Analysis and Mitigation of Software Applications'' \cite{reganoProlog}. It is organized in the following sections:

% \begin{itemize}
% 	\item Section~\ref{sec:prolog:app} describes the preliminary of the application structure modeling in the inference engine, previously obtained by \esp parsing the source code;
% 	\item Section~\ref{sec:prolog:goals} defines the rules needed to model the attacker goals;
% 	\item Section~\ref{sec:prolog:att} details the methodology for modelling attack steps, and how the inference engine combines them in attack paths;
% 	\item Section~\ref{sec:prolog:risk} reports on the method used to assess the risk of the inferred attack paths;
% 	\item Section~\ref{sec:prolog:validation} contains a comparison of the obtained results \wrt the \esp requisites defined in \ref{sec:esp:problem}.
% \end{itemize}

%At the start of the risk assessment phase, the \esp models all the information regarding the application structure in form of Prolog axioms, \ie facts that the engine consider true by definition. Then, the \esp queries the engine to find, for each asset security requirement, a sequence of rules (\ie attack steps) that, given the aforementioned axioms, can prove the breach of an asset security requirement. Attack paths will thus start with an attack step having only preconditions on the applic

%given the aforementioned axioms, to infer all the possible logical sequences of rules that can lead to the


\subsubsection{Application structure modeling}
\label{sec:prolog:app}

\begin{itemize}
    \item application, code, datum facts
    \item relationships facts (containment, call graph)
    \item asset + security requirements facts
\end{itemize}

% This section presents the modelling of all the preliminary information needed by the inference engine to find possible attacks against the application, comprising assets with their security requirements and the application structure. All this information is automatically retrieved by \esp in the preliminary source code analysis phase of its workflow.

% First, the existence of an application $a$ is defined with the following fact:
% \begin{equation*}
% \infer{application(a)}{}
% \end{equation*}
% Then, the application structure must be formally modelled. Each basic component of the code can be either a code or a datum (a constant or a variable); for example, if the application $a$ contains a function $f$ and a global variable $d$, this can be modelled with the following facts, using by abuse of notation the symbol $\rhd$ to indicate the containment relationship:
% \begin{equation*}
% \infer{code(f)}{} \quad \infer{datum(d)}{} \quad \infer{f \rhd a}{} \quad \infer{d \rhd a} {}
% \end{equation*}
% The containment relationship permits to organize the application structure in a hierarchical way. For example, if the function $c$ contains a local variable $v$, and a code snippet $s$, we can define the function structure with the following facts:
% \begin{equation*}
% \infer{datum(v)}{} \quad \infer{\rhd f}{} \quad \infer{code(s)}{} \quad \infer{\rhd f}{}
% \end{equation*}
% Then, a code $c$ accessing a variable $v$ can be expressed with the following fact:
% \begin{equation*}
% \infer{accesses(c,v)}{}
% \end{equation*}
% Also the call graph of the application can be modelled; if a function $f_1$ containing a call to a function $f_2$, the following fact holds:
% \begin{equation*}
% \infer{calls(f_1,f_2)}{}
% \end{equation*}
% Finally, the assets and their security requirements must be defined. If the \esp user requests the confidentiality security requirement \infer{\confidentiality}{} for a function $f_1$, integrity \infer{\integrity}{} for a function $f_2$ , and execution correctness \infer{\excorr}{} for a function $f_3$, the following facts are asserted:
% \begin{equation*}
% \infer{code(f_1)}{} \quad \infer{code(f_2)}{} \quad \infer{code(f_3)}{} \quad
% \infer{\confidentiality(f_1)}{} \quad \infer{\integrity(f_2)}{} \quad \infer{\excorr(f_3)}{}
% \end{equation*}

\subsubsection{Attacker goals modeling}
\label{sec:prolog:goals}

\begin{itemize}
    \item goal = breach asset security requirement
    \item basic rules to reach breaching of each of 3 sec. req.
\end{itemize}

% After modelling the application structure, and the assets with their security requirement, the basic rules that define the goals of the attacker can be defined. \esp, for each asset security requirement, will query the inference engine to find a set of rules that lead to breaching the requirement, denoted formally as the logical negation of the requirement. For example, if the application contains a variable $v$ whose confidentiality must be safeguarded, the inference engine will try to find all the possible sequences of attack steps that lead to the following outcome, which is a goal $G$ of the attacker:
% \begin{equation}
% \neg \confidentiality(v) \iff G.
% \end{equation}

% Security requirements are characterized by the different ways in which the attacker can breach them. The confidentiality of an asset $a_1$ is breached if the attacker finds a way to retrieve its content (instructions if $a_1$ is a code, or data if $a_1$ is a variable): 
% \begin{equation*}
% \infer{\neg \confidentiality(a_1)}{contentRetrieved(a_1)}
% \end{equation*}
% The integrity of an asset $a_2$ is breached if the attacker manages to change it, modelled with the following rules:
% \begin{equation*}
% \infer{\neg \integrity(a_2)}{changed(y)}
% \end{equation*}
% To model the breaching of execution correctness, two rules are needed. Formally, the attacker breaches the execution correctness of a code, either by modifying its instructions, or by avoiding the execution of the code, removing at least one call to the function. Thus, if a function $f$ is marked with the execution correctness requirement, the latter can be modelled with the following rules:
% \begin{equation}
% \infer{\neg \excorr(f)}{changed(f)} \quad \infer{\neg \excorr(f)}{calls(g,f) & changed(g)}
% \end{equation}
% With the definition of the following facts in the inference engine, \esp informs the latter of the application structure and of the security requirements of the assets. Thus, the attacks able reach the attacker goals, \ie to breach the security requirements of the assets, will adapt to the application structure.

\subsubsection{Attack steps and paths modeling}
\label{sec:prolog:att}

\begin{itemize}
    \item just 1 example of attack tree building
    \item ref to more complex examples in SPRO+WISTP papers
    \item brief description of actual implementation
    \item complexity analysis
\end{itemize}

% This section elaborates on the formal modelling of attack steps, basic and indivisible tasks that an attacker may carry out, and that can be combined into complete attack paths against the application assets. 

% %For the purpose of this section, it is sufficient to mark each attack step with a general id $AS$, to distinguish them from regular inference rules. Indeed, this distinction is important for the \esp: attack steps identify actions executed by the attacker, which can be deferred in the risk mitigation phase, while regular rules are simple inferences used to connect logically attack steps together, but with no use in the aforementioned phase. Also, when presenting inferred attack paths to the user, including normal inferences would result in unnecessary clutter that would complicate user comprehension of the paths.

% First, a set of basic attack steps must be defined. First, the attacker may retrieve the content of a hard-coded asset $h$, \eg a constant or a set of instructions, by locating it in the binary, and inspecting the latter manually:
% \begin{equation*}
% \infer[statLocate(h)]{contentRetrieved(h)}{hardcoded(h)}
% \end{equation*}

% Conversely, the attacker may retrieve the instructions constituting a code asset $c$ at run-time, for example by means of step-by-step execution with a debugger, provided that the execution flow of the application can lead to the target code. Similarly, an attacker can read the value of a local variable $v$ locating it in memory at run-time. This leads to the following attack steps:
% \begin{equation*}
% \infer[dynLocate(c)]{contentRetrieved(c)}{code(c)}
% \end{equation*}
% \begin{equation*}
% \infer[dynLocate(v)]{contentRetrieved(v)}{datum(v) & v \rhd f }
% \end{equation*}

% If an attacker wants to locate a datum $d$ to retrieve its value, he may try to first identify and execute at run-time a function $f$ that uses the aforementioned datum, thus finding it in memory when the instruction of the function $f$ that accesses the datum $d$ is executed:
% \begin{equation*}
% \infer[dynLocate(d)]{contentRetrieved(d)}{code(c) & contentRetrieved(c) & accesses(c,v)    }
% \end{equation*}
% Also, if an attacker wants to locate a function $f$, and he or she has already retrieved a function $g$ that calls $f$, then by simply following the call, looking at the target address of the call instruction, he or she can retrieve the function $f$ in the binary:
% \begin{equation*}
% \infer[followCall(g,f)]{contentRetrieved(f)}{calls(g,f) & contentRetrieved(g)}
% \end{equation*}
% Thus, if such datum $d$ is a confidential asset, one of the possible attack paths, leading to the attacker goal $G$ of breaching $d$ confidentiality can be obtained by chaining the previous attack steps:
% \begin{equation*}
% \infer{G}{
% 	\infer{\neg \confidentiality(d)}{
% 		\infer[dynLocate(d)]{contentRetrieved(d)}{
% 			\infer[statLocate(c)]{contentRetrieved(c)}{\infer{hardcoded(c)}{\infer{code(c)}{}}} & \infer{accesses(c,v)}{}
% 		}
% 	}
% }
% \end{equation*}
% % In this example, the attacker first identifies the address of the function $c$ in the code section of the application binary, analyzing statically the latter. Indeed the $statLocate(c)$ attack step can be executed, because $c$, being a code, is hard-coded. Then he or she attaches a debugger to the application and sets a breakpoint at the address of the function $c$ previously located. Then, since the code $c$ accesses the variable $v$, by executing $c$ step-by-step the attacker is able to find the variable $v$ when $c$ accesses it, and thus, knowing $v$'s location in memory, can retrieve its content. Therefore, the confidentiality of the asset $d$ is breached, and the attacker goal $G$ is proved. Clearly, instead of this hybrid approach (\ie by resorting to both static and dynamic analysis), the attacker can breach $d$ confidentiality in a completely dynamic manner, finding the code $c$ observing the execution flow of the application. Similarly, the call graph of the application can be used to define other attack steps. For example, an attacker may locate a function $f_1$ at run-time, if he has previously located a function $f_2$ that calls $f_1$, and the function is executed.

% % For tampering attacks two types of attack steps may be modelled. As for the retrieval of content, tampering may be carried out statically only on hard-coded assets, while it can be executed dynamically on every kind of asset. Given a code or datum $x$, the attacker may change it statically or dynamically with the following attack steps, which require the attacker to know the location of $x$:
% % \begin{equation*}
% % \infer[statChange(x)]{changed(x)}{contentRetrieved(x) & hardcoded(x)} 
% % \end{equation*}
% % \begin{equation*}
% % \infer[dynChange(x)]{changed(x)}{contentRetrieved(x)}
% % \end{equation*}

% % Thus, attack paths that endanger the integrity and execution correctness security requirements of an asset can be obtained by chaining the steps required to locate the asset that must be tampered, and the steps in which the attacker actually tamper with the asset. Given a function $f$ whose execution correctness must be preserved, \ie $f$ must not be tampered with, and all the calls to $f$ must be executed, this attacker goal $G$ can be obtained with the following two example attack paths:
% % \begin{equation*}
% % \infer{G}{
% % 	\infer{\neg \excorr(f)}{
% % 		\infer{calls(g,f)}{} & \infer[statChange(g)]{changed(g)}{  \infer[statLocate(g)]{contentRetrieved(g)}{\infer{hardcoded(g)}{}}      }
% % 	}                            
% % }
% % \end{equation*}
% % \begin{equation*}
% % \infer{G}{
% % 	\infer{\neg \excorr(f)}{
% % 		\infer[dynChange(f)]{changed(f)}{\infer[followCall(g,f)]{contentRetrieved(f)}{\infer{calls(g,f)}{} &
% % 				\infer[statLocate(g)]{contentRetrieved(g)}{\infer{hardCoded(g)}{}}
% % 		}}
% % 	}
% % }
% % \end{equation*}
% % In the first attack path, the attacker first locates the function $g$. He can do it statically since $g$ is hard-coded. Then he or her changes it, removing from $g$ the call to the asset $f$. In this way, the execution correctness of $f$ is broken. In the second attack path, the attacker locates statically the function $g$ as before, but in this case uses its address to set a breakpoint in a debugger attached to the application. For example, this can be useful in the case of an indirect call, when the target address of the call (\ie the address of $f$) is not known a priori, since it is evaluated by the program at run-time. Thus, he will execute the application, which will stop at the breakpoint set at the start of function $g$. With an execution step-by-step of the function $g$, the attacker finds the call to function $f$, follows it an then retrieves the address of the address function, thus being able to change the contained instructions and breach the execution correctness of the asset $f$.

% % Thus, starting from apparently naive attack steps, the inference engine can combine them in rather complex attack paths. All the concept and relationships among them, modelling the application structure, are obtained automatically by \esp, thus these attack paths can be obtained in a completely automated fashion, with the users asked only for the security requirements of the assets.

% Other attack steps have been devised to model attacks on applications that include network connections in their execution flow, modelling sniffing, spoofing and remote code injection attacks. However, these attack steps cannot be employed in a completely automated workflow by \esp, since it would require the identification of the specific functions that perform such network activity. This is complicated to do automatically, especially if the application uses custom network libraries. Since the requirements for \esp (see Section~\ref{sec:esp:problem}) state that all workflow phases must be executed automatically, such network-based attack steps are not deemed relevant for the scope of this thesis. Still, use of the spoofing attack step to model attacks against an \otp generator has been reported in a conference publication \cite{basileOTP}.

% The chaining of the rules is executed by the inference engine via a custom backward programming algorithm, called by \esp for each asset security requirement. Given this goal, the algorithm starts by negating the asset security requirement and then finds all the possible attack steps that can lead to the asset security requirement negation: each parallel attack step leads to a separate attack path. Then, it goes on building all the possible paths: for each of the latter, the algorithm consider completely inferred a path when the last attack step requirements can be proved only with the axioms detailing the application. Therefore, \esp builds for each asset security requirement an attack graph, which contains four different attack paths to breach the execution correctness of a code $c_2$, which is called by another function $c_1$.

% %as the one depicted in Figure~\ref{fig:attackGraph}\footnote{The avoidedCalls fact has been added to the graph to ease comprehension, but would not be present in a real attack path.},
% %\tikzstyle{Function} = [rectangle,rounded corners,draw=black, top color=white,
% %bottom color=white!50,very thick, inner sep=0.4em, minimum size=1.5em, text
% %centered]
% %\tikzstyle{Variable} = [rectangle,draw=black, top color=white, bottom
% %color=white!50,very thick, inner sep=0.4em, minimum size=1.5em, text centered]
% %\tikzstyle{myarrow} = [->, >=latex', shorten >=1pt, thick]
% %\tikzstyle{mydashedarrow} = [->, >=latex', shorten >=1pt, dashed]
% %\tikzstyle{mythickarrow} = [->, >=latex', shorten >=1pt,line width=0.6mm]
% %\tikzstyle{mylabel} = [text width=7em, text centered]
% %
% %\begin{figure}[t]
% %\centering
% %\begin{tikzpicture}[node distance=0.3cm, auto]
% %\node [Function] (breached) {breached(executionCorrectness,$c_2$)};
% %\node [Function, above right = of {$(breached)+(+0.6,+0.5)$}]
% %(changedC2)
% %{changed($c_2$)};
% %\node [Variable, above right = of {$(changedC2)+(+1.5,-0.1)$}]
% %(statChC2)
% %{statChange($c_2$)};
% %\node [Variable, right = of {$(statChC2)+(+1.511,0)$}]
% %(statLocC2)
% %{statLocate($c_2$)};
% %\node [Variable, below right = of {$(changedC2)+(+1.5,+0.1)$}]
% %(dynChC2)
% %{dynChange($c_2$)};
% %\node [Variable, right = of {$(dynChC2)+(+1.511,0)$}]
% %(dynLocC2)
% %{dynLocate($c_2$)};
% %\node [Function, below right = of {$(breached)+(-0.4,-0.4)$}]
% %(avoided)
% %{avoidedCalls($c_2$)};
% %\node [Function, below right = of {$(avoided)+(-0.6,-0.4)$}]
% %(changedC1)
% %{changed($c_1$)};        
% %\node [Variable, above right = of {$(changedC1)+(+1.5,-0.1)$}]
% %(stChC1)
% %{statChange($c_1$)};
% %\node [Variable, right = of {$(stChC1)+(+1.511,0)$}]
% %(statLocC1)
% %{statLocate($c_1$)};
% %\node [Variable, below right = of {$(changedC1)+(+1.5,+0.1)$}]     
% %(dynChC1)
% %{dynChange($c_1$)};
% %\node [Variable, right = of {$(dynChC1)+(+1.511,0)$}]
% %(dynLocC1)
% %{dynLocate($c_1$)};
% %
% %\draw[mydashedarrow] ($(avoided.north)+(-0.1,0)$) --
% %(breached.south);    
% %\draw[mydashedarrow] (changedC1.north) -- (avoided.south);    
% %\draw[mydashedarrow] (changedC2.south) -- (breached.north);    
% %\draw[myarrow] (dynChC1.west) --
% %($(changedC1.east)+(-0.08,-0.2)$);
% %\draw[myarrow] (stChC1.west) --
% %($(changedC1.east)+(-0.08,+0.2)$);\draw[myarrow]
% %(dynChC2.west) --
% %($(changedC2.east)+(-0.08,-0.2)$);
% %\draw[myarrow] (statChC2.west) --
% %($(changedC2.east)+(-0.08,+0.2)$);
% %\draw[mythickarrow] (statLocC2.west) -- (statChC2.east);
% %\draw[mythickarrow] (dynLocC2.west) -- (dynChC2.east);
% %\draw[mythickarrow] (statLocC1.west) -- (stChC1.east);
% %\draw[mythickarrow] (dynLocC1.west) -- (dynChC1.east);
% %
% %\end{tikzpicture}
% %\caption{Attack graph built against the execution correctness of a code $c2$, which is called by the code $c1$.}
% %\label{fig:attackGraph}
% %\end{figure}

% %\subsection{Network attack steps}
% %\label{sec:prolog:network}
% %This section models two additional attack steps, modelling sniffing and spoofing attacks, thus being suitable to assess threats on applications that, during their execution, communicate with a remote server. For example, e-banking websites typically employ a two-factor authentication: to access its account, and every time it executes a security-sensitive operation (\eg a money transfer to another bank account), the user must not only provide its credentials, but also a \otp, valid only to authorize a single operation. \glspl{otp} are typically generated either using a hardware dongle, or with a mobile application. In the second case, the \otp is generation is based on a pre-shared secret among the mobile application and the e-banking server, and on a factor that changes every time a new \otp is requested by the user: for example, a counter that is incremented every time a new \otp is generated. An attacker, which has already stolen the access credentials of a user, may be interested in being able to generate such passwords at will, hacking the \otp generator. 
% %%
% %To help with the modelling of this network attack steps, the \otp example is used throughout the section, thus is needed to describe its execution flow. At the first installation on the e-banking service user device, the \otp generator downloads two random values from the server, using an encrypted connection: a \textit{seed} and a \textit{counter}. Then, every time the user requests a new \otp, the generator asks a \pin to the user, so that unauthorized users having gained access (\eg stealing) to the device running the generator can obtain access to the e-banking account of the user. If the \pin inserted is correct, the generator produces the \otp, with a method based on the values of the aforementioned seed and counter, which is known to both the application and the e-banking server; thus, the \otp inserted by the user when accessing the e-banking site can be validated against the \otp produced on the server with the same method and the same values of seed and counter. After the generation of the \otp, the counter is incremented both on the generator and on the server, and a new \otp can be produced. 



\subsubsection{Risk probability}
\label{sec:prolog:risk}

\begin{itemize}
    \item evaluation of risk of each attack path on unprotected application
    \item useful for expert manual assessment of proposed L1P solution
    \item not used by automatic risk mitigation phase (since risks are on unprotected app)
    \item formulas (already present on WISTP paper, maybe just a ref is sufficient)
\end{itemize}

% In this section, a method to assess the probability of the threats against the application assets is presented. \esp, when presenting the attack paths to the user, includes also such a  probability: this is useful for experts that want to manually analyze the protections inferred by \esp in the risk mitigation phase, since they can identify the assets that are most at risk, and consequently focus on the protections targeting the most threatened assets.

% Instead, it will not be used to drive the risk mitigation phase (see Section~\ref{sec:l1p:metrics:score}): the motivation behind this is that the probabilities inferred in this phase refer to the unprotected application, while the risk mitigation phase uses a set of formulas tailored to assess the effect of attacks on protected assets, to assess the effectiveness of the inferred mitigations.

% The risk probability is based on the types of attacks inferred, and on the presumed skills of the attacker, given the profile chosen by the user at the start of the \esp workflow. Given all the inferred attack paths \(AP_{i}\), all their attack steps \(AS_{i,j}\), and all the assets \(a_{k}\), the \emph{risk} $\Omega_{\mathrm{AP}_{i}}^\epsilon$ of an attack path \(AP_{i}\) executed by an attacker with expertise $\epsilon$ is defined as:
% \begin{equation*}
% \Omega_{\mathrm{AP}_{i}}^\epsilon = \pi(\mathrm{AP}_{i},\epsilon)\;\Gamma_{\mathrm{AP}_{i}}\;\label{eq:risk}
% \end{equation*}
% where $\Gamma_{\mathrm{AP}_{i}}$ represents the damage resulting from a successful attack path, and  $\pi({\mathrm{AP}_{i}},\epsilon)$ is the probability of an attacker being able to successfully carry out the attack path, given its expertise $\epsilon$. To do so, it must be able to execute all the attack steps needed to complete it. Thus, the probability of executing an attack path is evaluated taking into account the probabilities of all the attack steps constituting the path:
% \begin{equation*}
% \pi({\mathrm{AP}_{i}},\epsilon) = f\left(\pi({\mathrm{AS}_{i,1}},\epsilon),\pi({\mathrm{AS}_{i,2}},\epsilon),\dots\right).
% \end{equation*}
% The \esp user can decide the function $f$ that must be used to combine the probabilities of the attack steps belonging to the same path, choosing among a worst case analysis, with $f=min$, a best case analysis, with $f=max$, and an approximation of the probabilities composition, with $f=\cdot$.

% $\Gamma_{\mathrm{AP}_{i}}$ is a quantitative measure of the damage resulting from a successful attack path. It is evaluated as the sum of the damage $\Gamma_{\mathrm{AS}_{i,j}}$ from each attack step:
% \[
% \Gamma_{\mathrm{AP}_{i}} = \sum_j \Gamma_{\mathrm{AS}_{i,j}}= \sum_j \sum_{k} ( W_{a_{k}} b( a_{k},\mathrm{AS}_{i,j}) )
% \]
% %where $\Gamma_{\mathrm{AS}_{i,j}}$  is the cost of a single attack step
% where \(W_{a_{k}}\) is a user-defined asset weight, and \(b( a_{k},\mathrm{AS}_{j})\) is a function, evaluated by \esp, that returns the fraction of the security properties of the asset \(a_{k}\) that are breached by the attack step \(\mathrm{AS}_{j}\), that is, it returns \(1\) if all the security properties are compromised and \(0\) if none\footnote{Thus, the whole asset weight assigned by the user is gained by the attacker when all the security properties are compromised.}.
% %\(b( a_{k},\mathrm{AS}_{j})\) is .

% The attack step probabilities $\pi({\mathrm{AS}_{i,j}})$, for each combination of attack step type, and level of attacker skill, have been obtained during the \asp project, interviewing the software security experts involved in the project during \esp design phase.


% %
% %The \esp employs a worst case analysis, setting $f=min$, thus the probability of an attack path is approximated as the one of the most easy attack step. 
% %
% %$\Gamma_{\mathrm{AP}_{i}}$ is a quantitative measure of the damage resulting from a successful attack path, calculated as the sum of the damage $\Gamma_{\mathrm{AS}_{i,j}}$ from each attack step:
% %
% %\[
% %\Gamma_{\mathrm{AP}_{i}} = \sum_j \Gamma_{\mathrm{AS}_{i,j}}= \sum_j \sum_{k} ( W_{a_{k}} b( a_{k},\mathrm{AS}_{i,j}) )
% %\]
% %%where $\Gamma_{\mathrm{AS}_{i,j}}$  is the cost of a single attack step
% %where \(W_{a_{k}}\) is the user-defined asset weight, and \(b( a_{k},\mathrm{AS}_{j})\) is a function, deduced by our inference system, which returns the fraction of the security properties of the asset \(a_{k}\) that are breached by the attack step \(\mathrm{AS}_{j}\), which is, it returns \(1\) if all the security properties are compromised and \(0\) if none\footnote{In practice, we assume that the whole asset weight assigned by the user is gained by the attacker when all the security properties are compromised.}. Finally, the values obtained with the risk formulas are mapped on a three values score (low, medium, high) with an ad hoc mapping.

\subsubsection{Validation}
\label{sec:prolog:validation}

\begin{itemize}
    \item cite requirements, why they are solved and why we are so cool
\end{itemize}

% In this section, the methodologies presented in this chapter, used by \esp to infer possible attack paths against the application assets, are compared \wrt the \esp requisites listed in Section~\ref{sec:esp:problem}.

% Regarding the requisites on the usage scenario of \esp, detailed in Sec.~\ref{sec:esp:problem:framing}, they are satisfied by the risk assessment phase. First, the profile of the attacker is taken into account, when the risk of each attack path is evaluated. Second, the execution of the backward programming algorithm used by the inference engine can be constrained, using a hard time limit, and also setting a maximum length for the attack paths: a deeper and more time-consuming search is suitable prior to the distribution of the application, while, when patches are released and time is an issue, a shallow search for possible new attack paths derived from the introduction of the patch code can be performed, limiting the time needed using the aforementioned constraints. Third, the results of the mitigation phase, \ie attack paths, are easily readable, being modelled as ordered sequences of simple attack steps: furthermore, logical inferences that do not correspond to real tasks executed by the attacker are not included in the paths, to avoid confusion for the user. Furthermore, a risk level for each inferred attack path is presented to the \esp user, which can easily identify the most problematic threats to the application.

% Analyzing the requisites for the risk assessment phase, described in Sec.~\ref{sec:esp:problem:assessment}, they are mostly satisfied. First, \esp supports not only the security requirements defined by the \nist for risk monitoring \cite{nistSP800-39}, \ie confidentiality and integrity, but also a stronger form of the latter, called execution correctness, and applicable only to functions: this security requirement prescribes that the function marked with it must not only be preserved from modification, but it must be also called as originally devised by the application developer (\eg a license check that must not be circumvented). Furthermore, \esp is able to build attack graphs for every asset in the application, due to the definition of logical inference rules that define attack steps, \ie simple attacker tasks. The chaining of these steps in attack paths is subject to the application structure, which is automatically modelled with logical facts in the inference engine: thus, the relative requirement is satisfied. Finally, a probability of execution for each attack path is evaluated, based on the attacker skills, and the probability of execution of each attack step: the latter are based on information gathered among the software security experts involved in the \asp project. The complexity metrics of the software are not taken into account in the attack path probability evaluation: however, they are taken into account later in the \esp workflow, during the risk mitigation phase, when the effectiveness of the inferred protections in protecting the assets, against the attack path inferred in the risk assessment phase, is tested with a game-theoretic approach based on this metrics.

% Finally, in the validation phase of \esp at the end of the \asp project \cite{D1.06.9}, software security experts analyzed also the attack paths inferred in the risk mitigation phase. In particular, the ones inferred by \esp on the \asp use cases (see Section~\ref{sec:esp:results}) were compared with actual attacks executed by highly skilled white-hat hackers on the same test applications. In general, \esp attack paths covered the real methodologies of the aforementioned hackers. However, they were deemed as too general to model with a sufficient amount of detail such attacks. Indeed, new rules can be added to the inference engine, in order to better model real attacks on software: however, as in the case of network-related attacks, the main problem is inferring automatically the semantics of the code that enables the execution of such complex attack step. Thus, this is still an open problem, which the author is actively investigating, in particular focusing on automated binary exploitation frameworks \cite{angr, huang}, which could be used to actually assess the vulnerabilities of the applications in an automated manner. Their results could be still modelled as attack paths, thus being compatible with the remainder of the workflow.

==> contributions.tex <==
model of assets, attacks, protections, security properties, etc.
and their dependencies
to find attack paths and suitable protections
game theoretic algorithm to identify solutions
heuristics to prune the search space
backward reasoning to find attack paths
already declared in publications
evaluation models to estimate impact of attack paths and protections
metrics composition
metrics change estimation after protections
L2P
Minor
integration with the ACTC
GUI
reports that are validated by experts


==> discussion.tex <==
threats to validity/limitations/validation vs. requirements for each workflow step

\begin{itemize}
\item Knowledge base
\item Risk assessment
\begin{itemize}
    \item discuss why we analyze the vanilla version
    \item difficulties (i.e. why coarse attack steps = backward programming combinatorial explosion + no way to automatically model actual attack steps)
    \item validation vs. requirements
\end{itemize}
\item Asset protection: ref to analogous subsection in section IV
\item Asset hiding
\begin{itemize}
        \item excessive AH may decrease AP solution security level
        \item overhead
        \item AH refines a AP solution thus all AP difficulties also apply to AH
\end{itemize}
\end{itemize}

==> main_bbl.tex <==
\begin{thebibliography}{100}
\providecommand{\url}[1]{{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{DOI~\discretionary{}{}{}#1}\else
  \providecommand{\doi}{DOI~\discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url}\fi

\bibitem{CWE-656}
{CWE-656}: Reliance on security through obscurity.
\newblock \url{https://cwe.mitre.org/data/definitions/656.html}

\bibitem{magicquadrant}
{Gartner Magic Quadrant for Network Firewalls}.
\newblock \url{https://www.gartner.com/en/documents/4007809}

\bibitem{owl2}
Owl 2 web ontology language new features and rationale (second edition).
\newblock W3c recommendation, World Wide Web Consortium (W3C), Cambridge, MA,
  US (2012).
\newblock \urlprefix\url{https://www.w3.org/TR/owl2-new-features/}

\bibitem{frost}
Global software licensing and monetization market, forecast to 2021.
\newblock Tech. Rep. 3715874, Frost \& Sullivan (2016)

\bibitem{ENISA}
{ENISA good practices for security of Smart Cars}.
\newblock Tech. rep., {European Union Agency for Cyber Security} (2019)

\bibitem{10.1145/2229156.2229157}
van~der Aalst, W.: Process mining: Overview and opportunities.
\newblock ACM Trans. Manage. Inf. Syst. \textbf{3}(2) (2012).
\newblock \doi{10.1145/2229156.2229157}

\bibitem{renewability}
Abrath, B., Coppens, B., Van~den Broeck, J., Wyseur, B., Cabutto, A., Falcarin,
  P., De~Sutter, B.: Code renewability for native software protection.
\newblock ACM Transactions on Privacy and Security \textbf{23}(4) (2020)

\bibitem{circulardebugging}
Abrath, B., Coppens, B., Nevolin, I., De~Sutter, B.: Resilient self-debugging
  software protection.
\newblock In: 2020 IEEE European Symposium on Security and Privacy Workshops,
  pp. 606--615. IEEE Computer Society (2020)

\bibitem{diabloSelfDebugging}
Abrath, B., Coppens, B., Volckaert, S., Wijnant, J., De~Sutter, B.:
  Tightly-coupled self-debugging software protection.
\newblock In: Proc.\ of the 6th Workshop on Software Security, Protection, and
  Reverse Engineering (SSPREW), pp. 7:1--7:10. ACM (2016)

\bibitem{ahmadvand2018}
Ahmadvand, M., Pretschner, A., Kelbert, F.: A taxonomy of software integrity
  protection techniques.
\newblock Advances in Computers  (2019).
\newblock \doi{https://doi.org/10.1016/bs.adcom.2017.12.007}

\bibitem{MATEtaxonomy}
Akhunzada, A., Sookhak, M., Anuar, N.B., Gani, A., Ahmed, E., Shiraz, M.,
  Furnell, S., Hayat, A., {Khurram Khan}, M.: Man-at-the-end attacks: Analysis,
  taxonomy, human aspects, motivation and future directions.
\newblock Journal of Network and Computer Applications \textbf{48}, 44--57
  (2015).
\newblock \doi{https://doi.org/10.1016/j.jnca.2014.10.009}

\bibitem{Anckaert2006}
Anckaert, B., Jakubowski, M., Venkatesan, R.: Proteus: Virtualization for
  diversified tamper-resistance.
\newblock In: Proceedings of the ACM Workshop on Digital Rights Management, p.
  47–58. ACM (2006)

\bibitem{Anckaert2007}
Anckaert, B., Madou, M., De~Sutter, B., De~Bus, B., De~Bosschere, K., Preneel,
  B.: Program obfuscation: a quantitative approach.
\newblock In: Proc.\ 2007 ACM workshop on Quality of Protection, pp. 15--20
  (2007)

\bibitem{Ban17}
Banescu, S., Collberg, C., Pretschner, A.: Predicting the resilience of
  obfuscated code against symbolic execution attacks via machine learning.
\newblock In: Proc.\ 26th USENIX Security Symposium, pp. 661--678 (2017)

\bibitem{banescu2017tutorial}
Banescu, S., Pretschner, A.: A tutorial on software obfuscation.
\newblock In: Advances in Computers, vol. 108, pp. 283--353. Elsevier (2017).
\newblock \doi{10.1016/bs.adcom.2017.09.004}

\bibitem{barakImpossibility}
Barak, B., Goldreich, O., Impagliazzo, R., Rudich, S., Sahai, A., Vadhan, S.,
  Yang, K.: On the (im)possibility of obfuscating programs.
\newblock In: J.~Kilian (ed.) Advances in Cryptology, pp. 1--18. Springer
  Berlin Heidelberg (2001)

\bibitem{basileOTP}
Basile, C., Canavese, D., d'Annoville, J., De~Sutter, B., Valenza, F.:
  Automatic discovery of software attacks via backward reasoning.
\newblock In: Proc.\ 1st Int'l Workshop on Software Protection, SPRO '15, pp.
  52--58. IEEE Press (2015)

\bibitem{D1.06}
Basile, C., Canavese, D., Regano, L.: {ASPIRE Validation}.
\newblock In: ASPIRE Project Deliverable 1.06 (2016).
\newblock
  \urlprefix\url{https://aspire-fp7.eu/sites/default/files/D1.06-ASPIRE-Validation-v1.01.pdf}

\bibitem{reganoMeta}
Basile, C., Canavese, D., Regano, L., Falcarin, P., De~Sutter, B.: A meta-model
  for software protections and reverse engineering attacks.
\newblock Journal of Systems and Software \textbf{150}, 3--21 (2019)

\bibitem{D5.11}
Basile, C., et~al.: {ASPIRE Framework Report}.
\newblock Deliverable D5.11, {ASPIRE EU FP7 Project} (2016).
\newblock
  \urlprefix\url{https://aspire-fp7.eu/sites/default/files/D5.11-ASPIRE-Framework-Report.pdf}

\bibitem{ceccato-new-one}
Berlato, S., Ceccato, M.: A large-scale study on the adoption of anti-debugging
  and anti-tampering protections in android apps.
\newblock Journal of Information Security and Applications \textbf{52}, 102,463
  (2020)

\bibitem{AESwhite}
Bringer, J., Chabanne, H., Dottax, E.: White box cryptography: Another attempt.
\newblock Cryptology ePrint Archive, Report 2006/468 (2006)

\bibitem{JENS}
Van~den Broeck, J., Coppens, B., De~Sutter, B.: Obfuscated integration of
  software protections.
\newblock Int'l Journal of Information Security \textbf{20}, 73--101 (2021)

\bibitem{brumley_apeg}
Brumley, D., Poosankam, P., Song, D., Zheng, J.: Automatic patch-based exploit
  generation is possible: Techniques and implications.
\newblock In: IEEE Symposium on Security and Privacy, pp. 143 -- 157. IEEE
  Computer Society (2008)

\bibitem{10.1145/3338503.3357722}
Brunet, P., Creusillet, B., Guinet, A., Martinez, J.M.: Epona and the
  obfuscation paradox: Transparent for users and developers, a pain for
  reversers.
\newblock In: Proceedings of the 3rd ACM Workshop on Software Protection, pp.
  41--52. Association for Computing Machinery (2019)

\bibitem{BSA}
{BSA | The Software Alliance}: {BSA Global Software Piracy Survey}.
\newblock Online at \url{https://gss.bsa.org/} (2018)

\bibitem{bsimm}
{Building Security in Maturity Model}.
\newblock \urlprefix\url{https://www.bsimm.com/}

\bibitem{mckinsey-automotive}
Burkacky, O., Deichmann, J., Klein, B., Pototzky, K., Scherf, G.: Cybersecurity
  in automotive.
\newblock Tech. rep., McKinsey \& Company (2020)

\bibitem{codeMobility}
Cabutto, A., Falcarin, P., Abrath, B., Coppens, B., De~Sutter, B.: Software
  protection with code mobility.
\newblock In: Proc.\ of the 2nd ACM Workshop on Moving Target Defense, MTD '15,
  pp. 95--103. ACM (2015)

\bibitem{reganoMetric}
Canavese, D., Regano, L., Basile, C., Viticchi{\'e}, A.: Estimating software
  obfuscation potency with artificial neural networks.
\newblock In: Security and Trust Management, pp. 193--202. Springer
  International Publishing (2017)

\bibitem{D4.06}
Ceccato, M.: {ASPIRE Security Evaluation Methodology}.
\newblock Deliverable D4.06, {ASPIRE EU FP7 Project} (2016)

\bibitem{barrierslicing}
Ceccato, M., Dalla~Preda, M., Nagra, J., Collberg, C., Tonella, P.: Barrier
  slicing for remote software trusting.
\newblock In: 7th IEEE Int'l Working Conference on Source Code Analysis and
  Manipulation (SCAM), pp. 27--36. IEEE Computer Society (2007)

\bibitem{ceccatoTaxonomy}
Ceccato, M., Tonella, P., Basile, C., Coppens, B., De~Sutter, B., Falcarin, P.,
  Torchiano, M.: How professional hackers understand protected code while
  performing attack tasks.
\newblock In: 2017 IEEE/ACM 25th International Conference on Program
  Comprehension (ICPC), pp. 154--164. IEEE Computer Society (2017)

\bibitem{emse2019}
Ceccato, M., Tonella, P., Basile, C., Falcarin, P., Torchiano, M., Coppens, B.,
  De~Sutter, B.: Understanding the behaviour of hackers while performing attack
  tasks in a professional setting and in a public challenge.
\newblock Empirical Software Engineering \textbf{24}(1), 240--286 (2019)

\bibitem{chow2002white}
Chow, S., Eisen, P., Johnson, H., van Oorschot, P.C.: A white-box {DES}
  implementation for {DRM} applications.
\newblock In: J.~Feigenbaum (ed.) Digital Rights Management, pp. 1--15.
  Springer Berlin Heidelberg (2003)

\bibitem{DSRA-evaluation-alternatives}
Cleven, A., Gubler, P., H\"{u}ner, K.M.: Design alternatives for the evaluation
  of design science research artifacts.
\newblock In: Proc.\ 4th Int'l Conf.\ on Design Science Research in Information
  Systems and Technology, DESRIST '09. Association for Computing Machinery, New
  York, NY, USA (2009).
\newblock \doi{10.1145/1555619.1555645}

\bibitem{tigress}
Collberg, C., Martin, S., Myers, J., Nagra, J.: Distributed application tamper
  detection via continuous software updates.
\newblock In: Proc.\ of the 28th Annual Computer Security Applications
  Conference, p. 319–328. ACM (2012)

\bibitem{collberg1997taxonomy}
Collberg, C., Thomborson, C., Low, D.: A taxonomy of obfuscating
  transformations.
\newblock Computer Science Technical Reports 148, Dep.\ of Computer Science,
  University of Auckland, New Zealand (1997)

\bibitem{collbergOpake}
Collberg, C., Thomborson, C., Low, D.: Manufacturing cheap, resilient, and
  stealthy opaque constructs.
\newblock In: Proc.\ 25th ACM SIGPLAN-SIGACT symposium on Principles of
  programming languages, pp. 184--196 (1998)

\bibitem{coppens2013feedback}
Coppens, B., De~Sutter, B., Maebe, J.: Feedback-driven binary code
  diversification.
\newblock ACM Transactions on Architecture and Code Optimization (TACO)
  \textbf{9}(4), 1--26 (2013)

\bibitem{D5.13}
Coppens, B., et~al.: {ASPIRE Open Source Manual}.
\newblock Deliverable D5.13, {ASPIRE EU FP7 Project} (2016).
\newblock
  \urlprefix\url{https://aspire-fp7.eu/sites/default/files/D5.13-ASPIRE-Open-Source-Manual.pdf}

\bibitem{robust}
Dawes, R.M.: The robust beauty of improper linear models in decision making.
\newblock American psychologist \textbf{34}(7), 571 (1979)

\bibitem{AESbroken}
De~Mulder, Y., Wyseur, B., Preneel, B.:
  Cryptanalysis\,of\,a\,perturbated\,white-box\,{AES}\,implementation.
\newblock In: G.~Gong, K.C. Gupta (eds.) Progress in Cryptology-INDOCRYPT 2010,
  pp. 292--310. Springer Berlin Heidelberg (2010)

\bibitem{Dagstuhl}
{De Sutter}, B., Collberg, C., {Dalla Preda}, M., Wyseur, B.: {Software
  Protection Decision Support and Evaluation Methodologies (Dagstuhl Seminar
  19331)}.
\newblock Dagstuhl Reports \textbf{9}(8), 1--25 (2019)

\bibitem{nistir8011}
{Dempsey, Kelley and Takamura, Eduardo and Eavy, Paul and Moore, George}:
  {NISTIR 8011 Vol. 4. Automation Support for Security Control Assessments:
  Software Vulnerability Management.}
\newblock Tech. rep., National Institute of Standards \& Technology,
  Gaithersburg, MD, United States (2020)

\bibitem{idesReq}
Denning, D., Neumann, P.G.: Requirements and model for ides -- a real-time
  intrusion-detection expert system.
\newblock Tech. rep., SRI International, Menlo Park, CA, USA (1985)

\bibitem{doerry2015monetizing}
Doerry, N., Sibley, M.: Monetizing risk and risk mitigation.
\newblock Naval Engineers Journal \textbf{127}, 35--46 (2015)

\bibitem{GOP}
van~der Ende, M., Hageraats, M., Poort, J., Quintais, J.P., Yagafarova, A.:
  Global online piracy study 2018.
\newblock Online at
  \url{https://www.ivir.nl/projects/global-online-piracy-study/} (2018)

\bibitem{fwExpSys}
Eronen, P., Zitting, J.: An expert system for analyzing firewall rules.
\newblock In: Proceedings of the 6th Nordic Workshop on Secure IT Systems
  (NordSec 2001), pp. 100--107 (2001)

\bibitem{gdpr1yafter}
{European Union Agency for Fundamental Rights (FRA)}: The general data
  protection regulation -- one year on.
\newblock Tech. rep., {}European Union Agency for Fundamental Rights (FRA)
  (2019)

\bibitem{Gartner-report-riskanalysis}
{Gartner, Inc.}: Risk assessment process and methodologies primer for 2019.
\newblock Online at \url{https://www.gartner.com/en/documents/3938592} (2019)

\bibitem{Gartner-report-online}
{Gartner, Inc.}: Cybersecurity labor shortage and {COVID-19}.
\newblock Online at
  \url{https://www.gartner.com/en/human-resources/research/talentneuron/cybersecurity-labor-shortage-and-covid-19}
  (2020)

\bibitem{heffner2004obfuscation}
Heffner, K., Collberg, C.: The obfuscation executive.
\newblock In: K.~Zhang, Y.~Zheng (eds.) Information Security, pp. 428--440.
  Springer Berlin Heidelberg, Berlin, Heidelberg (2004)

\bibitem{hevner2004design}
Hevner, A.R., March, S.T., Park, J., Ram, S.: Design science in information
  systems research.
\newblock MIS quarterly pp. 75--105 (2004)

\bibitem{hoffman1986risk}
Hoffman, L.J.: Risk analysis and computer security: bridging the cultural gaps.
\newblock In: Proceedings of the 9th National Computer Security Conference, pp.
  156--161. National Institute of Standards and Technology (1986)

\bibitem{obf_evaloptphaseord}
Holder, W., McDonald, J.T., Andel, T.R.: Evaluating optimal phase ordering in
  obfuscation executives.
\newblock In: Proc.\ 7th Software Security, Protection, and Reverse Engineering
  Workshop, SSPREW-7. ACM (2017)

\bibitem{horvath2020cryptographic}
Horv{\'a}th, M., Butty{\'a}n, L.: Cryptographic Obfuscation: A Survey.
\newblock Springer (2020)

\bibitem{Irdeto-report1}
Irdeto: Irdeto global connected industries cybersecurity survey.
\newblock Online at
  \url{https://go.irdeto.com/connected-industries-cybersecurity-survey-report/}
  (2020)

\bibitem{ISO27k}
{Information technology - Security techniques - Information security management
  systems - Overview and vocabulary}.
\newblock Standard, International Organization for Standardization,
  International Electrotechnical Commission, Geneva, CH (2018)

\bibitem{ISO27004}
{Information technology - Security techniques - Information security management
  - Monitoring, measurement, analysis and evaluation}.
\newblock Standard, International Organization for Standardization,
  International Electrotechnical Commission (2016)

\bibitem{nistSP800-37}
{Joint Task Force}: {SP 800-37}. risk management framework for information
  systems and organizations (revision 2).
\newblock Tech. rep., National Institute of Standards \& Technology,
  Gaithersburg, MD, United States (2018)

\bibitem{nistSP800-53}
{Joint Task Force}: {SP 800-53}. security and privacy controls for information
  systems and organizations (revision 5).
\newblock Tech. rep., National Institute of Standards \& Technology,
  Gaithersburg, MD, United States (2020)

\bibitem{nistSP800-39}
{Joint Task Force Transformation Initiative}: {SP 800-39}. managing information
  security risk: Organization, mission, and information system view.
\newblock Tech. rep., National Institute of Standards \& Technology (2011)

\bibitem{thinking}
Kahneman, D.: Thinking, fast and slow.
\newblock Macmillan (2011)

\bibitem{conditions}
Kahneman, D., Klein, G.: Conditions for intuitive expertise: a failure to
  disagree.
\newblock American psychologist \textbf{64}(6), 515 (2009)

\bibitem{intro_crypto}
Kaltz, J., Lindell, Y.: Introduction to modern cryptography: principles and
  protocols.
\newblock Chapman and Hall  (2008)

\bibitem{knapsack-book}
Kellerer, H., Pferschy, U., Pisinger, U.: Knapsack Problems.
\newblock Springer-Verlag (2004)

\bibitem{Khanmohammadi2019repacked}
Khanmohammadi, K., Hamou-Lhadj, A., Ebrahimi, N., Khoury, R.: Empirical study
  of android repackaged applications.
\newblock {Empirical Software Engineering} \textbf{24}(6), 3587--3629 (2019)

\bibitem{kimForensics}
Kim, J.S., Kim, M., Noh, B.N.: A fuzzy expert system for network forensics.
\newblock In: Computational Science and Its Applications (ICCSA), pp. 175--182.
  Springer Berlin Heidelberg (2004)

\bibitem{arxan-report}
Knight, A.: In plain sight: The vulnerability epidemic in financial mobile apps
  (April 2019)

\bibitem{CPI}
Kuznetsov, V., Szekeres, L., Payer, M., Candea, G., Sekar, R., Song, D.:
  Code-pointer integrity.
\newblock In: 11th {USENIX} Symposium on Operating Systems Design and
  Implementation, pp. 147--163. {USENIX} Association (2014)

\bibitem{liaoForensics}
Liao, N., Tian, S., Wang, T.: Network forensics based on fuzzy logic and expert
  system.
\newblock Comput. Commun. \textbf{32}(17), 1881--1892 (2009)

\bibitem{linn2003branchFunctions}
Linn, C., Debray, S.: Obfuscation of executable code to improve resistance to
  static disassembly.
\newblock In: Proceedings 10th ACM conference on Computer and communications
  security, pp. 290--299. ACM, New York, NY, USA (2003)

\bibitem{obf_optvialangmods}
Liu, H.: Towards better program obfuscation: Optimization via language models.
\newblock In: Proc.\ 38th Int'l Conference on Software Engineering Companion,
  ICSE '16, pp. 680--682. Association for Computing Machinery (2016)

\bibitem{7985664}
Liu, H., Sun, C., Su, Z., Jiang, Y., Gu, M., Sun, J.: Stochastic optimization
  of program obfuscation.
\newblock In: Proceedings of the 39th International Conference on Software
  Engineering, ICSE '17, pp. 221--231. IEEE Press (2017)

\bibitem{lukyanenko2014instantiation}
Lukyanenko, R., Evermann, J., Parsons, J.: Instantiation validity in is design
  research.
\newblock In: Advancing the Impact of Design Science: Moving from Theory to
  Practice: 9th International Conference, DESRIST 2014, Miami, FL, USA, May
  22-24, 2014. Proceedings 9, pp. 321--328. Springer (2014)

\bibitem{instantiation-validity}
Lukyanenko, R., Evermann, J., Parsons, J.: Instantiation validity in is design
  research.
\newblock In: M.C. Tremblay, D.~VanderMeer, M.~Rothenberger, A.~Gupta, V.~Yoon
  (eds.) Advancing the Impact of Design Science: Moving from Theory to
  Practice, pp. 321--328. Springer International Publishing, Cham (2014)

\bibitem{10.1007/978-3-030-55583-2_9}
Macher, G., Schmittner, C., Veledar, O., Brenner, E.: {ISO/SAE DIS 21434}
  automotive cybersecurity standard - in a nutshell.
\newblock In: Proceedings of Computer Safety, Reliability, and Security
  (SAFECOMP) Workshops: DECSoS 2020, DepDevOps 2020, USDAI 2020, and WAISE
  2020, pp. 123–--135. Springer-Verlag (2020).
\newblock \doi{10.1007/978-3-030-55583-2_9}

\bibitem{Mandiant}
Mandiant: 2020 security effectiveness: Deep dive into cyber reality.
\newblock Online at
  \url{https://content.fireeye.com/security-effectiveness/rpt-security-effectiveness-2020-deep-dive-into-cyber-reality}
  (2020)

\bibitem{ReMind}
Mantovani, A., Aonzo, S., Fratantonio, Y., Balzarotti, D.: {RE-Mind}: a first
  look inside the mind of a reverse engineer.
\newblock In: Proc. 32st Usenix Security Symposium (2022).
\newblock To appear

\bibitem{mccabe}
McCabe, T.J.: A complexity measure.
\newblock IEEE Transactions on Software Engineering \textbf{SE-2}(4), 308--320
  (1976)

\bibitem{merlo2021repackage}
Merlo, A., Ruggia, A., Sciolla, L., Verderame, L.: You shall not repackage!
  demystifying anti-repackaging on android.
\newblock Computers and Security \textbf{103}, 102,181 (2021)

\bibitem{collbergbook}
Nagra, J., Collberg, C.: Surreptitious Software: Obfuscation, Watermarking, and
  Tamperproofing for Software Protection.
\newblock Pearson Education, London, UK (2009)

\bibitem{rational}
Osbeck, L.M., Held, B.S.: Rational intuition: Philosophical roots, scientific
  investigations.
\newblock Cambridge University Press (2014)

\bibitem{owaspasvs}
{OWASP Application Security Verification Standard v4.03} (2021).
\newblock
  \urlprefix\url{https://owasp.org/www-project-application-security-verification-standard/}

\bibitem{owaspsamm}
{OWASP Software Assurance Maturity Model v2.0} (2020).
\newblock \urlprefix\url{https://owaspsamm.org/}

\bibitem{owensIDS}
Owens, S.F., Levary, R.R.: An adaptive expert system approach for intrusion
  detection.
\newblock Int. J. Secur. Netw. \textbf{1}(3/4), 206--217 (2006)

\bibitem{attack_graphs}
Phillips, C., Swiler, L.P.: A graph-based system for network-vulnerability
  analysis.
\newblock In: Proceedings of the 1998 Workshop on New Security Paradigms, NSPW
  ’98, pp. 71--79. ACM (1998)

\bibitem{Prat-taxonomy}
Prat, N., Comyn-Wattiau, I., Akoka, J.: A taxonomy of evaluation methods for
  information systems artifacts.
\newblock Journal of Management Information Systems \textbf{32}(3), 229--267
  (2015).
\newblock \doi{10.1080/07421222.2015.1099390}

\bibitem{ReganoPhd}
Regano, L.: An expert system for automatic software protection.
\newblock Ph.D. thesis, Politecnico di Torino (2019)

\bibitem{reganoL2P}
Regano, L., Canavese, D., Basile, C., Lioy, A.: Towards optimally hiding
  protected assets in software applications.
\newblock In: Proc.\ Int'l Conf.\ on Software Quality, Reliability and
  Security, pp. 374--385. IEEE Computer Society (2017)

\bibitem{reganoProlog}
Regano, L., Canavese, D., Basile, C., Viticchi{\'e}, A., Lioy, A.: Towards
  automatic risk analysis and mitigation of software applications.
\newblock In: Information Security Theory and Practice, pp. 120--135. Springer
  International Publishing (2016)

\bibitem{virtualizationAttack}
Rolles, R.: Unpacking virtualization obfuscators.
\newblock In: Proceedings of the 3rd USENIX Conference on Offensive
  Technologies, WOOT'09, pp. 1--1. USENIX Association (2009)

\bibitem{schrittwieser2016}
Schrittwieser, S., Katzenbeisser, S., Kinder, J., Merzdovnik, G., Weippl, E.:
  Protecting software through obfuscation: Can it keep pace with progress in
  code analysis?
\newblock ACM Comput. Surv. \textbf{49}(1), 4:1--4:37 (2016)

\bibitem{angr}
Shoshitaishvili, Y., Wang, R., Salls, C., Stephens, N., Polino, M., Dutcher,
  A., Grosen, J., Feng, S., Hauser, C., Kruegel, C., Vigna, G.: Sok: (state of)
  the art of war: Offensive techniques in binary analysis.
\newblock In: 2016 IEEE Symposium on Security and Privacy (SP), pp. 138--157.
  IEEE Computer Society (2016)

\bibitem{nistSP800-40}
{Souppaya, Murugiah and Scarfone, Karen}: {SP 800-40 Rev.~4. Guide to
  Enterprise Patch Management Planning: Preventive Maintenance for Technology}.
\newblock Tech. rep., National Institute of Standards \& Technology (2017)

\bibitem{Tamada2012}
Tamada, H., Fukuda, K., Yoshioka, T.: Program incomprehensibility evaluation
  for obfuscation methods with queue-based mental simulation model.
\newblock In: 13th ACIS Int'l Conf.\ on Software Engineering, Artificial
  Intelligence, Networking and Parallel Distributed Computing, pp. 498--503
  (2012)

\bibitem{standardization}
Tassey, G.: Standardization in technology-based markets.
\newblock Research policy \textbf{29}(4-5), 587--602 (2000)

\bibitem{RevEngE}
Taylor, C., Collberg, C.: Getting {RevEngE}: a system for analyzing reverse
  engineering behavior.
\newblock In: 14th International Conference on Malicious and Unwanted Software
  ({MALCON}) (2019)

\bibitem{audes}
Tsudik, G., Summers, R.C.: Audes - an expert system for security auditing.
\newblock In: Proceedings of the The Second Conference on Innovative
  Applications of Artificial Intelligence, pp. 221–--232. AAAI Press (1990)

\bibitem{architectural}
Tuma, K., Calikli, G., Scandariato, R.: Threat analysis of software systems: A
  systematic literature review.
\newblock Journal of Systems and Software \textbf{144}, 275--294 (2018)

\bibitem{Jens2}
{Van den Broeck}, J., Coppens, B., {De Sutter}, B.: Flexible software
  protection.
\newblock Computers \& Security \textbf{116}, 102,636 (2022)

\bibitem{diablo}
{Van Put}, L., Chanet, D., {De Bus}, B., {De Sutter}, B., {De Bosschere}, K.:
  {DIABLO}: a reliable, retargetable and extensible link-time rewriting
  framework.
\newblock In: Proc.\ Fifth IEEE Int'l Symposium on Signal Processing and
  Information Technology, pp. 7--12. IEEE Computer Society (2005)

\bibitem{FEDS-evaluation}
Venable, J., Pries-Heje, J., Baskerville, R.: {FEDS}: a framework for
  evaluation in design science research.
\newblock European Journal of Information Systems \textbf{25}(1), 77--89
  (2016).
\newblock \doi{10.1057/ejis.2014.36}

\bibitem{viticchie2016reactive}
Viticchi\'{e}, A., Basile, C., Avancini, A., Ceccato, M., Abrath, B., Coppens,
  B.: Reactive attestation: Automatic detection and reaction to software
  tampering attacks.
\newblock In: Proceedings of the 2016 ACM Workshop on Software PROtection, SPRO
  '16, p. 73–84. ACM (2016)

\bibitem{wangFlatteningTechReport}
Wang, C., Hill, J., Knight, J., Davidson, J.: Software tamper resistance:
  Obstructing static analysis of programs.
\newblock Tech. rep., University of Virginia, Charlottesville, VA, USA (2000)

\bibitem{petri_nets_attacks}
Wang, H., Fang, D., Wang, N., Tang, Z., Chen, F., Gu, Y.: Method to evaluate
  software protection based on attack modeling.
\newblock In: Int'l Conf.\ on High Performance Computing and Communications
  (HPCC) \& Int'l Conf.\ on Embedded and Ubiquitous Computing (EUC), pp.
  837--844. IEEE Computer Society (2013)

\bibitem{SWI-Prolog}
Wielemaker, J., Schrijvers, T., Triska, M., Lager, T.: {SWI-Prolog}.
\newblock Theory and Practice of Logic Programming \textbf{12}(1-2), 67--96
  (2012)

\bibitem{OWASPrisk}
Williams, J.: {OWASP Risk Rating Methodology}.
\newblock Online at
  \url{https://owasp.org/www-community/OWASP_Risk_Rating_Methodology} (1930)

\bibitem{wohlin00}
Wohlin, C., Runeson, P., H\"ost, M., Ohlsson, M., Regnell, B., Wessl\'en, A.:
  Experimentation in Software Engineering - An Introduction.
\newblock Kluwer Academic Publishers (2000)

\bibitem{wyseur2011white}
Wyseur, B.: White-box cryptography.
\newblock Ph.D. thesis, KU Leuven (2011)

\bibitem{D1.02}
Wyseur, B.: Assets.
\newblock In: ASPIRE Project Deliverable 1.02: Attack Model, pp. 10--12 (2014)

\bibitem{D1.02attack}
Wyseur, B.: Classification of attacks.
\newblock In: ASPIRE Project Deliverable 1.02: Attack Model, pp. 13--52 (2014)

\bibitem{DESbroken}
Wyseur, B., Michiels, W., Gorissen, P., Preneel, B.: Cryptanalysis of white-box
  {DES} implementations with arbitrary external encodings.
\newblock In: C.~Adams, A.~Miri, M.~Wiener (eds.) Selected Areas in
  Cryptography, pp. 264--277. Springer Berlin Heidelberg (2007)

\bibitem{yadegari}
Yadegari, B., Johannesmeyer, B., Whitely, B., Debray, S.: A generic approach to
  automatic deobfuscation of executable code.
\newblock In: Proc.\ Symposium on Security and Privacy, pp. 674–--691. IEEE
  Computer Society (2015)

\bibitem{Zhou2012repacked}
Zhou, Y., Jiang, X.: Dissecting android malware: Characterization and
  evolution.
\newblock In: 2012 IEEE Symposium on Security and Privacy, pp. 95--109 (2012).
\newblock \doi{10.1109/SP.2012.16}

\bibitem{Gartner}
Zumerle, D., Bhat, M.: Gartner: Market guide for application shielding (2017)

\end{thebibliography}


==> pkgnumcompress.tex <==
%%
%% This is file 'numcompress'.
%%
%% Copyright (C) 2009-2012 River Valley Technologies 
%%                    <latex.support@river-valley.com>
%%   
%% This package may be distributed under the terms of the LaTeX Project 
%% Public License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
%% $Id: numcompress.sty 187 2012-08-18 09:36:35Z rishi $
%% $URL: http://lenova.river-valley.com/svn/elsbst/trunk/numcompress.sty $
%%
\NeedsTeXFormat{LaTeX2e}
\def\Fileversion$#1: #2 ${\gdef\fileversion{#2}}
\def\Filedate$#1: #2-#3-#4 #5 #6 #7 ${\gdef\filedate{#2/#3/#4}} 
\Fileversion$Rev: 187 $
\Filedate$LastChangedDate: 2012-08-18 15:06:35 +0530 (Sat, 18 Aug 2012) $
\ProvidesPackage{numcompress}
   [\filedate\space\fileversion\space numcompress (CVR)]
\PackageWarningNoLine{numcompress}
   {****************************************\MessageBreak
    Package numcompress v,\fileversion\space loaded\MessageBreak
    [Compress numbers (CVR)]\MessageBreak
    ****************************************}
\newif\ifdots \dotsfalse
\newif\ifnumcompress \numcompresstrue

\DeclareOption{dots}{\global\dotstrue}
\DeclareOption{nodots}{\global\dotsfalse}
\DeclareOption{compress}{\global\numcompresstrue}
\DeclareOption{nocompress}{\global\numcompressfalse}

\ProcessOptions 

\def\removeDot#1{\def\tmp{#1}%
    \ifx\tmp\@empty\else\@removeDot#1\@nil\fi}

\def\@removeDot#1\@nil{\edef\fchar{\expandafter\@car#1\@nil}%
      \edef\rchar{\expandafter\@cdr#1!\@nil}%
      \def\@xmltempa{.}\def\@xmltempb{!}%
      \ifx\fchar\@xmltempb\relax\else%
      \ifx\fchar\@xmltempa\relax\else%
      \fchar\ignorespaces\fi\removeDot{\rchar}\fi}

\def\First[#1]{\csname First#1\endcsname}
\def\Second[#1]{\csname Second#1\endcsname}

\def\parseFirstPage#1{\@tempcnta=0
  \@tfor\@digits:=#1\do{%
    {\global\advance\@tempcnta by 1
      \expandafter\xdef\csname
      First\the\@tempcnta\endcsname{\@digits}%
      \xdef\flength{\the\@tempcnta}}}}

\def\parseSecondPage#1{\@tempcnta=0
  \@tfor\@digits:=#1\do{%
    {\global\advance\@tempcnta by 1
      \expandafter\xdef\csname
      Second\the\@tempcnta\endcsname{\@digits}%
      \xdef\llength{\the\@tempcnta}}}}

\newif\ifdissimilar\dissimilarfalse
\def\checkequal#1#2{\edef\Farg{#1}\edef\Sarg{#2}%
      \edef\One{A}%
      \ifcat\One\Farg \relax\else%
      \ifdissimilar\Sarg\else%
      \ifnum\Farg=\Sarg\relax\else\Sarg\dissimilartrue\fi\fi\fi}
%
\let\@@fpage\@empty
\let\@@lpage\@empty
\def\fpage@compress#1{%
      \gdef\@@fpage{#1}%
            \edef\llength{0}%
            \parseFirstPage{#1}%
      \ifnum\flength=\llength%
       \gdef\@fpage{\@@fpage}%
       \gdef\@lpage{%
        \@ifundefined{Second1}{}{\checkequal{\First[1]}{\Second[1]}}%
        \@ifundefined{Second2}{}{\checkequal{\First[2]}{\Second[2]}}%
        \@ifundefined{Second3}{}{\checkequal{\First[3]}{\Second[3]}}%
        \@ifundefined{Second4}{}{\checkequal{\First[4]}{\Second[4]}}%
        \@ifundefined{Second5}{}{\checkequal{\First[5]}{\Second[5]}}%
      }%
      \else%
       \gdef\@fpage{\@@fpage}%
       \gdef\@lpage{\@@lpage}%
     \fi}

\def\lpage@compress#1{%
        \gdef\@@lpage{#1}%
        \parseSecondPage{#1}%
      \ifnum\flength=\llength%
       \gdef\@fpage{\@@fpage}%
       \gdef\@lpage{%
       \edef\One{A}%
       \edef\xFirst{\First[1]}%
       \edef\xSecond{\Second[1]}%
       \ifcat\One\xSecond\relax%
          \ifx\xFirst\xSecond%
           \@ifundefined{Second1}{}{\checkequal{\First[1]}{\Second[1]}}%
           \@ifundefined{Second2}{}{\checkequal{\First[2]}{\Second[2]}}%
           \@ifundefined{Second3}{}{\checkequal{\First[3]}{\Second[3]}}%
           \@ifundefined{Second4}{}{\checkequal{\First[4]}{\Second[4]}}%
           \@ifundefined{Second5}{}{\checkequal{\First[5]}{\Second[5]}}%
          \else#1\fi%
      \else%
          \ifx\xFirst\xSecond%
           \@ifundefined{Second1}{}{\checkequal{\First[1]}{\Second[1]}}%
           \@ifundefined{Second2}{}{\checkequal{\First[2]}{\Second[2]}}%
           \@ifundefined{Second3}{}{\checkequal{\First[3]}{\Second[3]}}%
           \@ifundefined{Second4}{}{\checkequal{\First[4]}{\Second[4]}}%
           \@ifundefined{Second5}{}{\checkequal{\First[5]}{\Second[5]}}%
        \else#1\fi%
      \fi%
      }%
    \else
      \gdef\@fpage{\@@fpage}%
      \gdef\@lpage{%
      \edef\Targ{#1}%
      \edef\One{A}%
      \edef\xFirst{\First[1]}%
      \edef\xSecond{\Second[1]}%
      \ifx\xFirst\xSecond
         \ifcat\One\xSecond\relax\else\@@lpage\fi%
      \else#1\fi%
      }%
  \fi}

%\newwrite\xx
%\immediate\openout\xx=tmpbib.tex
\gdef\@@lpage@compress#1--#2\@nil{\lpage@compress{#1}}
\gdef\@@@pages#1#2{\def\next{#2}%
%  \immediate\write\xx{[\the\c@NAT@ctr.]\space [#1][#2]}%
  \fpage@compress{#1}%\ifx\next\@empty\relax\else
   \@@lpage@compress#2\@nil%\fi
  {\@fpage\ifx\next\@empty\relax\else
    --\@lpage\fi}\resetall}

\gdef\@@@page#1{#1\resetall}

\def\mk@empty#1{\@tempcnta=1
  \loop\ifnum\@tempcnta<6
    \expandafter\let\csname#1\the\@tempcnta\endcsname\relax
    \advance\@tempcnta by 1 \repeat}
\def\resetall{\let\@lpage\@empty\let\@fpage\@empty
   \def\flength{0}\def\llength{0}%
   \let\@@fpage\@empty\let\@@lpage\@empty
   \mk@empty{First}\mk@empty{Second}}


\ifdots
 \gdef\xfnm[#1]{\unskip\space#1}
 \def\bibinfo#1#2{\@ifnextchar.{\@@bibinfo{#1}{#2}}{\@@@bibinfo{#1}{#2}}}
 \def\@@@bibinfo#1#2{\def\next{#1}%
   \def\@@@pg{pages}\def\@@@au{author}%
   \ifx\next\@@@pg\bibpages{#2}\else
   \ifx\next\@@@au\bibauthor{#2}\else
   #2\fi\fi}
 \def\@@bibinfo#1#2.{\def\next{#1}%
  \def\@@@pg{pages}\def\@@@au{author}%
  \ifx\next\@@@pg\bibpages{#2}.\else
  \ifx\next\@@@au\bibauthor{#2}\else
  #2.\fi\fi}
\else
 \gdef\xfnm[#1]{\unskip\space\removeDot{#1}}
 \def\bibinfo#1#2{\def\next{#1}%
   \def\@@@pg{pages}\def\@@@au{author}%
   \ifx\next\@@@pg\bibpages{#2}\else
   \ifx\next\@@@au\bibauthor{#2}\else
   #2\fi\fi}
\fi

\ifnumcompress
 \def\bibpages#1{\@@bibpages#1--\\\@nil}
 \def\@@bibpages#1--#2\@nil{%
   \ifx\\#2\relax\@@@page{#1}\else
   \@@@pages{#1}{#2}\fi}
 \else
 \def\bibpages#1{#1}
\fi

\def\bibauthor#1{#1}

\endinput

%%
%% End of package 'numcompress.sty'
%%


==> pkgpicins.tex <==
%       PICINS.STY --- Style File zum Einbinden von Bildern
%       Autor:  J. Bleser, E. Lang
%       Hochschulrechenzentrum
%       Technische Hochschule Darmstadt
%       !!!  Dieses Style-File ist urheberrechtlich geschuetzt  !!!
%       !!!  Aenderungen nur mit Zustimmung der Autoren         !!!
\message{Option `picins' Version 3.0  Sep. 1992, TH Darmstadt/HRZ}
\newbox\@BILD%
\newbox\@TEXT%
\newdimen\d@breite%
\newdimen\d@hoehe%
\newdimen\d@xoff%
\newdimen\d@yoff%
\newdimen\d@shad%
\newdimen\d@dash%
\newdimen\d@boxl%
\newdimen\d@pichskip%
\newdimen\d@tmp
\newdimen\d@tmpa
\newdimen\d@bskip
\newdimen\hsiz@%
\newdimen\p@getot@l%
\newcount\c@breite
\newcount\c@hoehe
\newcount\c@xoff
\newcount\c@yoff
\newcount\c@pos
\newcount\c@shad
\newcount\c@dash
\newcount\c@boxl
\newcount\c@zeilen%
\newcount\@changemode%
\newcount\c@piccaption%
\newcount\c@piccaptionpos%
\newcount\c@picpos
\newcount\c@whole%
\newcount\c@half%
\newcount\c@tmp
\newcount\c@tmpa
\newcount\c@tmpb
\newcount\c@tmpc
\newcount\c@tmpd
\newskip\d@leftskip
\newif\if@list \@listfalse%
\newif\if@offset%


\c@piccaptionpos=1%
\c@picpos=0
\d@shad=4pt%
\d@dash=4pt%
\d@boxl=10pt%
\d@pichskip=1em%
\@changemode=0%
\def\@captype{figure}%
\let\old@par=\par%

\def\pichskip#1{\d@pichskip #1\relax}


\def\shadowthickness#1{\d@shad #1\relax}


\def\dashlength#1{\d@dash #1\relax}


\def\boxlength#1{\d@boxl #1\relax}


\def\picchangemode{\@changemode=1}%
\def\nopicchangemode{\@changemode=0}%


\def\piccaptionoutside{\c@piccaptionpos=1}%
\def\piccaptioninside{\c@piccaptionpos=2}%
\def\piccaptionside{\c@piccaptionpos=3}%
\def\piccaptiontopside{\c@piccaptionpos=4}%

\def\piccaption{\@ifnextchar [{\@piccaption}{\@piccaption[]}}
\def\@piccaption[#1]#2{\c@piccaption=1\def\sh@rtf@rm{#1}\def\capti@nt@xt{#2}}
\def\make@piccaption{%
 \hsiz@\d@breite%
 \ifnum\c@piccaptionpos=2%
   \advance\hsiz@ -2\fboxsep%
 \fi%
 \ifnum\c@piccaptionpos>2%
   \hsiz@\hsize\advance\hsiz@-\d@breite\advance\hsiz@-\d@pichskip%
 \fi%
 \setbox\@TEXT=\vbox{\hsize\hsiz@\caption[\sh@rtf@rm]{\capti@nt@xt}}%
}



\def\newcaption{\refstepcounter\@captype\@dblarg{\@newcaption\@captype}}
\long\def\@newcaption#1[#2]#3{%
  \old@par%
  \addcontentsline{\csname ext@#1\endcsname }{#1}%
    {\protect\numberline{\csname the#1\endcsname}{\ignorespaces #2}}
  \begingroup\@parboxrestore\normalsize%
    \@newmakecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\old@par%
  \endgroup%
}
\long\def\@newmakecaption#1#2{%
  \vskip 10pt%
  \setbox\@tempboxa \hbox {#1: #2}%
  \ifdim \wd\@tempboxa >\hsize%
    \setbox0=\hbox{#1: }\dimen0=\hsize\advance\dimen0 by-\wd0
    \setbox1=\vtop{\hsize=\dimen0 #2}
    \hbox{\box0 \box1}
    \par
  \else \hbox to\hsize {\hfil \box \@tempboxa \hfil}
  \fi
}





\def\parpic{%
  \@ifnextchar ({\iparpic}{\iparpic(0pt,0pt)}
}
\def\iparpic(#1,#2){%
  \@ifnextchar ({\@offsettrue\iiparpic(#1,#2)}%
                {\@offsetfalse\iiparpic(#1,#2)(0pt,0pt)}
}
\def\iiparpic(#1,#2)(#3,#4){%
  \@ifnextchar [{\iiiparpic(#1,#2)(#3,#4)}{\iiiparpic(#1,#2)(#3,#4)[l]}
}
\def\iiiparpic(#1,#2)(#3,#4)[#5]{%
  \@ifnextchar [{\ivparpic(#1,#2)(#3,#4)[#5]}{\ivparpic(#1,#2)(#3,#4)[#5][]}
}
\def\ivparpic(#1,#2)(#3,#4)[#5][#6]#7{%
 \let\par=\old@par\par%
 \hangindent0pt\hangafter1%
 \setbox\@BILD=\hbox{#7}%
 \d@breite=#1\d@breite=\the\d@breite%
 \ifdim\d@breite=0pt\d@breite=\wd\@BILD\fi%
 \c@breite=\d@breite\divide\c@breite by65536%
 \multiply\c@piccaption\c@piccaptionpos%
 \d@hoehe=#2\d@hoehe=\the\d@hoehe%
 \ifdim\d@hoehe=0pt\d@hoehe=\ht\@BILD\advance\d@hoehe by\dp\@BILD\fi%
 \c@hoehe=\d@hoehe\divide\c@hoehe by65536%
 \d@xoff=#3\c@xoff=\d@xoff\divide\c@xoff by65536%
 \d@yoff=\d@hoehe%
 \advance\d@yoff by-#4\c@yoff=\d@yoff\divide\c@yoff by65536%
 \c@pos=1\unitlength1pt%
 \if@offset%
   \setbox\@BILD=\hbox{%
     \begin{picture}(\c@breite,\c@hoehe)%
       \put(0,0){\makebox(\c@breite,\c@hoehe){}}%
       \put(\c@xoff,\c@yoff){\box\@BILD}%
     \end{picture}%
   }%
 \else%
   \setbox\@BILD=\hbox{%
     \begin{picture}(\c@breite,\c@hoehe)%
       \put(0,0){\makebox(\c@breite,\c@hoehe)[#6]{\box\@BILD}}%
     \end{picture}%
   }%
 \fi%
 \ifnum\c@piccaption=2%
   \make@piccaption%
   \advance\d@hoehe\ht\@TEXT\advance\d@hoehe\dp\@TEXT%
   \c@hoehe=\d@hoehe\divide\c@hoehe by65536%
   \setbox\@BILD=\vbox{\box\@BILD\vspace{-5pt}%
                       \hbox{\hspace{\fboxsep}\box\@TEXT}%
                       \vspace{4pt}}%
 \fi%
 \@tfor\@tempa := #5\do{%
   \if\@tempa f\setbox\@BILD=\hbox{\Rahmen(\c@breite,\c@hoehe){\box\@BILD}}\fi%
   \if\@tempa s\setbox\@BILD=\hbox{\Schatten(\c@breite,\c@hoehe){\box\@BILD}}\fi%
   \if\@tempa o\setbox\@BILD=\hbox{\Oval(\c@breite,\c@hoehe){\box\@BILD}}\fi%
   \if\@tempa d\setbox\@BILD=\hbox{\Strich(\c@breite,\c@hoehe){\box\@BILD}}\fi%
   \if\@tempa x\setbox\@BILD=\hbox{\Kasten(\c@breite,\c@hoehe){\box\@BILD}}\fi%
   \if\@tempa l\c@pos=1\fi%
   \if\@tempa r\c@pos=2\fi%
 }%
 \ifnum\c@piccaption=1%
   \make@piccaption%
   \advance\d@hoehe\ht\@TEXT\advance\d@hoehe\dp\@TEXT%
   \c@hoehe=\d@hoehe\divide\c@hoehe by65536%
   \setbox\@BILD=\vbox{\box\@BILD\vspace{-5pt}\hbox{\box\@TEXT}\vspace{4pt}}%
 \fi%
 \ifodd\count0\c@picpos=0\else\c@picpos=\@changemode\fi%
 \pagetotal=\the\pagetotal%
 \d@tmp=\pagegoal\advance\d@tmp by-\pagetotal\advance\d@tmp by-\baselineskip%
 \ifdim\d@hoehe>\d@tmp%
   \vskip 0pt plus\d@hoehe\relax\pagebreak[3]\vskip 0pt plus-\d@hoehe\relax%
   \ifnum\c@picpos=1\c@picpos=0\else\c@picpos=\@changemode\fi%
 \fi%
 \ifnum\c@picpos=1\ifnum\c@pos=1\c@pos=2\else\c@pos=1\fi\fi%
 \ifnum\@listdepth>0
   \@listtrue\parshape 0%
   \advance\hsize -\rightmargin%
   \d@leftskip \leftskip%
   \leftskip \@totalleftmargin%
   \if@inlabel\rule{\linewidth}{0pt}\vskip-\baselineskip\relax\fi%
 \else\@listfalse\medskip%
 \fi%
 \if@list\d@tmpa=\linewidth\else\d@tmpa=\hsize\fi%
 \ifnum\c@piccaption=3%
   \make@piccaption%
   \d@tmp\ht\@TEXT\advance\d@tmp\dp\@TEXT%
   \ifdim\d@hoehe>\d@tmp%
     \setbox\@TEXT=\vbox to\d@hoehe{\vfill\box\@TEXT\vspace{.2\baselineskip}\vfill}%
   \else%
     \setbox\@BILD=\vbox to\d@tmp{\vfill\box\@BILD\vfill}%
     \d@hoehe\d@tmp%
   \fi%
 \fi%
 \ifnum\c@piccaption=4%
   \make@piccaption%
   \d@tmp\ht\@TEXT\advance\d@tmp\dp\@TEXT%
   \setbox\@TEXT=\vbox to\d@hoehe{\vspace{-10pt}\box\@TEXT\vfil}%
   \advance\d@hoehe-\d@tmp%
 \fi%
 \ifnum\c@pos=1\d@tmpa=0pt%
   \ifnum\c@piccaption>2%
      \setbox\@BILD=\hbox{\box\@BILD\hspace{\d@pichskip}\hbox{\box\@TEXT}}%
   \fi%
 \else\advance\d@tmpa by-\wd\@BILD\d@breite=-\d@breite%
   \ifnum\c@piccaption>2%
      \d@tmpa=0pt%
      \setbox\@BILD=\hbox{\hbox{\box\@TEXT}\hspace{\d@pichskip}\box\@BILD}%
   \fi%
 \fi%
 \p@getot@l\the\pagetotal%
 \d@bskip\d@hoehe\advance\d@bskip by\parskip\advance\d@bskip by.3\baselineskip%
 {\noindent\hspace*{\d@tmpa}\relax%
  \box\@BILD\nopagebreak\vskip-\d@bskip\relax\nopagebreak}%
 \d@tmp=-\d@hoehe\divide\d@tmp by\baselineskip%
 \c@zeilen=\d@tmp\advance\c@zeilen by-1%
 \ifdim\d@breite<0pt\advance\d@breite by-\d@pichskip%
 \else\advance\d@breite by\d@pichskip%
 \fi%
 \hangindent=\d@breite%
 \hangafter=\c@zeilen%
 \let\par=\x@par%
 \ifnum\c@piccaption=3%
    \hangindent0pt\hangafter1\let\par=\old@par%
    \vskip\d@hoehe\vskip.2\baselineskip%
 \fi%
 \c@piccaption=0%
}




\newdimen\ptoti
\newdimen\ptotii
\def\x@par{%
 \ptoti\pagetotal%
 \old@par%
 \ptotii\pagetotal%
 \ifdim\ptoti=\ptotii%
   \d@tmp\d@hoehe%
 \else%
   \d@tmp\baselineskip%
   \multiply\d@tmp by\prevgraf%
   \advance\d@tmp by\parskip%
   \global\advance\d@hoehe by-\d@tmp\d@tmp=\d@hoehe%
 \fi%
 \ifdim\d@hoehe>0pt%
   \divide\d@tmp by\baselineskip\c@zeilen=-\d@tmp\advance\c@zeilen by-1%
   \c@zeilen=\the\c@zeilen%
 \else\c@zeilen=0
 \fi
 \ifnum\c@zeilen<0\hangafter=\c@zeilen\hangindent=\d@breite%
 \else\let\par=\old@par%
   \hangindent 0pt%
   \leftskip \d@leftskip%
   \if@list\parshape \@ne \@totalleftmargin \linewidth%
     \advance\hsize \rightmargin%
   \fi%
 \fi%
}


\def\picskip#1{%
 \let\par=\old@par%
 \par%
 \pagetotal\the\pagetotal%
 \c@tmp=#1\relax%
 \ifnum\c@tmp=0%
   \d@tmp\baselineskip\multiply\d@tmp by\prevgraf\advance\d@tmp\parskip%
   \ifdim\p@getot@l<\pagetotal
     \advance\d@hoehe by-\d@tmp\advance\d@hoehe by1ex%
     \ifdim\d@hoehe>0pt\vspace*{\d@hoehe}\fi%
   \fi%
   \ifdim\p@getot@l=\pagetotal%
     \advance\d@hoehe by-\d@tmp\advance\d@hoehe by1ex%
     \ifdim\d@hoehe>0pt\vspace*{\d@hoehe}\fi%
   \fi%
 \else\hangafter=-\c@tmp\hangindent=\d@breite%
 \fi%
 \leftskip \d@leftskip%
 \if@list\parshape \@ne \@totalleftmargin \linewidth%
   \advance\hsize \rightmargin%
 \fi%
}






\def\hpic{%
  \@ifnextchar ({\ihpic}{\ihpic(0pt,0pt)}
}
\def\ihpic(#1,#2){%
  \@ifnextchar ({\@offsettrue\iihpic(#1,#2)}%
                {\@offsetfalse\iihpic(#1,#2)(0pt,0pt)}
}
\def\iihpic(#1,#2)(#3,#4){%
  \@ifnextchar [{\iiihpic(#1,#2)(#3,#4)}{\iiihpic(#1,#2)(#3,#4)[l]}
}
\def\iiihpic(#1,#2)(#3,#4)[#5]{%
  \@ifnextchar [{\ivhpic(#1,#2)(#3,#4)[#5]}{\ivhpic(#1,#2)(#3,#4)[#5][]}
}
\def\ivhpic(#1,#2)(#3,#4)[#5][#6]#7{%
  \setbox\@BILD=\hbox{#7}%
  \d@breite=#1\d@breite=\the\d@breite%
  \ifdim\d@breite=0pt\d@breite=\wd\@BILD\fi%
  \c@breite=\d@breite\divide\c@breite by65536%
  \d@hoehe=#2\d@hoehe=\the\d@hoehe%
  \ifdim\d@hoehe=0pt\d@hoehe=\ht\@BILD\advance\d@hoehe by\dp\@BILD\fi%
  \c@hoehe=\d@hoehe\divide\c@hoehe by65536%
  \d@xoff=#3\c@xoff=\d@xoff\divide\c@xoff by65536%
  \d@yoff=\d@hoehe%
  \advance\d@yoff by-#4\c@yoff=\d@yoff\divide\c@yoff by65536%
  \c@pos=0\d@tmpa=\parindent\parindent=0pt\unitlength1pt%
  \if@offset
    \setbox\@BILD=\hbox{%
      \begin{picture}(\c@breite,\c@hoehe)%
        \put(0,0){\makebox(\c@breite,\c@hoehe){}}%
        \put(\c@xoff,\c@yoff){\box\@BILD}%
      \end{picture}%
    }%
  \else%
    \setbox\@BILD=\hbox{%
      \begin{picture}(\c@breite,\c@hoehe)%
        \put(0,0){\makebox(\c@breite,\c@hoehe)[#6]{\box\@BILD}}%
      \end{picture}%
    }%
  \fi%
  \@tfor\@tempa := #5\do{%
    \if\@tempa f\setbox\@BILD=\hbox{\Rahmen(\c@breite,\c@hoehe){\box\@BILD}}\fi%
    \if\@tempa s\setbox\@BILD=\hbox{\Schatten(\c@breite,\c@hoehe){\box\@BILD}}\fi%
    \if\@tempa o\setbox\@BILD=\hbox{\Oval(\c@breite,\c@hoehe){\box\@BILD}}\fi%
    \if\@tempa d\setbox\@BILD=\hbox{\Strich(\c@breite,\c@hoehe){\box\@BILD}}\fi%
    \if\@tempa x\setbox\@BILD=\hbox{\Kasten(\c@breite,\c@hoehe){\box\@BILD}}\fi%
    \if\@tempa t\c@pos=1\fi%
    \if\@tempa b\c@pos=2\fi%
  }%
 \ifnum\c@pos=0\parbox{\d@breite}{\makebox[0cm]{}\\\box\@BILD\smallskip}\fi%
 \ifnum\c@pos=1\parbox[t]{\d@breite}{\makebox[0cm]{}\\\box\@BILD\smallskip}\fi%
 \ifnum\c@pos=2\parbox[b]{\d@breite}{\makebox[0cm]{}\\\box\@BILD\smallskip}\fi%
 \parindent=\d@tmpa%
}






\def\Rahmen(#1,#2)#3{%
  \c@whole=\@wholewidth\divide\c@whole by65536%
  \c@half=\@halfwidth\divide\c@half by65536%
  \c@tmpa=#1\advance\c@tmpa by\c@whole\advance\c@tmpa by\c@whole%
  \c@tmpb=#2\advance\c@tmpb by\c@whole\advance\c@tmpb by\c@whole%
  \begin{picture}(\c@tmpa,\c@tmpb)%
    \put(\c@whole,\c@half){\framebox(#1,#2){#3}}%
  \end{picture}%
  \global\advance\d@breite by2\@wholewidth%
  \global\advance\d@hoehe by2\@wholewidth%
}


\def\Schatten(#1,#2)#3{%
  \c@whole=\@wholewidth\divide\c@whole by65536%
  \c@half=\@halfwidth\divide\c@half by65536%
  \c@shad=\d@shad\divide\c@shad by65536%
  \c@tmp=\c@whole\advance\c@tmp by\c@whole\c@tmpd=\c@tmp%
  \advance\c@tmp by\c@shad%
  \advance\c@tmpd by#1%
  \advance\c@half by\c@shad%
  \c@tmpa=#1\advance\c@tmpa by\c@tmp%
  \c@tmpb=#2\advance\c@tmpb by\c@tmp%
  \begin{picture}(\c@tmpa,\c@tmpb)%
    \put(\c@whole,\c@half){\framebox(#1,#2){#3}}%
    \put(\c@shad,0){\rule{\c@tmpd pt}{\c@shad pt}}%
    \put(\c@tmpd,0){\rule{\c@shad pt}{#2 pt}}%
  \end{picture}%
  \global\advance\d@breite by2\@wholewidth\global\advance\d@breite by\d@shad%
  \global\advance\d@hoehe by2\@wholewidth\global\advance\d@hoehe by\d@shad%
}


\def\Oval(#1,#2)#3{%
  \@wholewidth=0.4pt%
  \c@tmpa=\the#1\divide\c@tmpa by2%
  \c@tmpb=\the#2\divide\c@tmpb by2%
  \begin{picture}(#1,#2)%
    \put(\c@tmpa,\c@tmpb){\oval(#1,#2)}%
    \put(0.4,0.4){#3}%
  \end{picture}%
  \global\advance\d@breite by1pt\global\advance\d@hoehe by1pt%
}


\def\Strich(#1,#2)#3{%
  \c@whole=\@wholewidth\divide\c@whole by65536%
  \c@half=\@halfwidth\divide\c@half by65536%
  \c@dash=\d@dash\divide\c@dash by65536%
  \c@tmp=\c@whole\advance\c@tmp by\c@whole%
  \c@tmpa=#1\advance\c@tmpa by\c@tmp%
  \c@tmpb=#2\advance\c@tmpb by\c@tmp%
  \c@tmpc=#1\advance\c@tmpc by\c@whole%
  \c@tmpd=#2\advance\c@tmpd by\c@whole%
  \begin{picture}(\c@tmpa,\c@tmpb)%
    \put(\c@half,\c@half){\dashbox{\c@dash}(\c@tmpc,\c@tmpd){#3}}%
  \end{picture}%
  \global\advance\d@breite by2\@wholewidth%
  \global\advance\d@hoehe by2\@wholewidth%
}


\def\Kasten(#1,#2)#3{%
  \@wholewidth=0.4pt%
  \c@boxl=\d@boxl\divide\c@boxl by65536\c@boxl=\the\c@boxl%
  \c@tmpa=#1\advance\c@tmpa by\c@boxl%
  \c@tmpb=#2\advance\c@tmpb by\c@boxl%
  \c@tmp=#2%
  \begin{picture}(\c@tmpa,\c@tmpb)%
    \put(0,\c@boxl){\framebox(#1,#2){#3}}%
    \put(\c@boxl,0){\line(-1,1){\c@boxl}}%
    \put(\c@boxl,0){\line(1,0){#1}\line(-1,1){\c@boxl}}%
    \put(\c@boxl,0){\put(#1,0){\line(0,1){\c@tmp}%
         \put(0,\c@tmp){\line(-1,1){\c@boxl}}}}%
  \end{picture}%
  \global\advance\d@breite by\d@boxl%
  \global\advance\d@hoehe by\d@boxl%
}





\newbox\env@box%
\newdimen\d@envdp
\newcount\c@hsize
\newcount\c@envdp
\newdimen\d@envb

\long\def\frameenv{\@ifnextchar [{\@frameenv}{\@frameenv[\textwidth]}}
\long\def\@frameenv[#1]{%
 \hsiz@=\textwidth  \textwidth=#1  \d@envb=#1
 \advance\textwidth by-2\@wholewidth
 \advance\textwidth by-2\fboxsep
 \hsize=\textwidth   \linewidth=\textwidth
 \setbox\env@box=\vbox\bgroup}%
\def\endframeenv{%
 \egroup%
 \hsize=\hsiz@  \textwidth=\hsiz@  \linewidth=\hsiz@
 \c@breite=\d@envb   \divide\c@breite by65536
 \advance\d@envb by-2\@wholewidth
 \c@hsize=\d@envb  \divide\c@hsize by65536%
 \d@envdp=\dp\env@box  \advance\d@envdp by\ht\env@box%
 \advance\d@envdp by2\fboxsep%
 \d@hoehe=\d@envdp   \advance\d@hoehe by2\@wholewidth
 \c@hoehe=\d@hoehe   \divide\c@hoehe by65536
 \c@envdp=\d@envdp   \divide\c@envdp by65536%
 \c@tmp=\@wholewidth \divide\c@tmp by65536
 \vskip\@wholewidth%
 \unitlength 1pt\noindent%
 \begin{picture}(\c@breite,\c@hoehe)(0,0)
   \put(\c@tmp,\c@tmp){\framebox(\c@hsize,\c@envdp){\box\env@box}}
 \end{picture}%
}



\long\def\shadowenv{\@ifnextchar [{\@shadowenv}{\@shadowenv[\textwidth]}}
\long\def\@shadowenv[#1]{%
 \hsiz@=\textwidth  \textwidth=#1  \d@envb=#1
 \advance\textwidth by-2\@wholewidth
 \advance\textwidth by-2\fboxsep
 \advance\textwidth by-\d@shad%
 \hsize=\textwidth   \linewidth=\textwidth
 \setbox\env@box=\vbox\bgroup}%
\def\endshadowenv{%
 \egroup
 \hsize=\hsiz@  \textwidth=\hsiz@  \linewidth=\hsiz@
 \d@tmpa=\d@envb
 \c@breite=\d@envb   \divide\c@breite by65536
 \advance\d@envb by-2\@wholewidth  \advance\d@envb by-\d@shad
 \c@hsize=\d@envb  \divide\c@hsize by65536%
 \d@envdp=\dp\env@box  \advance\d@envdp by\ht\env@box%
 \advance\d@envdp by2\fboxsep%
 \c@envdp=\d@envdp   \divide\c@envdp by65536%
 \d@hoehe=\d@envdp
 \advance\d@hoehe by2\@wholewidth  \advance\d@hoehe by\d@shad
 \c@hoehe=\d@hoehe    \divide\c@hoehe by65536
 \c@shad =\d@shad     \divide\c@shad  by65536
 \c@tmp=\@wholewidth  \divide\c@tmp by65536
 \advance\d@tmpa by-2\d@shad
 \c@xoff =\d@tmpa     \divide\c@xoff by65536
 \advance\c@xoff by\c@shad  \advance\c@xoff by-1
 \advance\d@envdp by\@wholewidth
 \vskip\@halfwidth
 \unitlength 1pt\noindent%
 \begin{picture}(\c@breite,\c@hoehe)(0,0)
    \put(\c@tmp,\c@shad){\framebox(\c@hsize,\c@envdp){\box\env@box}}
    \put(\c@shad,0){\rule{\d@tmpa}{\d@shad}}%
    \put(\c@xoff,0){\rule{\d@shad}{\d@envdp}}%
 \end{picture}%
 \vskip\@halfwidth
}


\long\def\dashenv{\@ifnextchar [{\@dashenv}{\@dashenv[\textwidth]}}
\long\def\@dashenv[#1]{%
 \hsiz@=\textwidth  \textwidth=#1  \d@envb=#1
 \advance\textwidth by-2\@wholewidth  \advance\textwidth by-2\fboxsep
 \hsize=\textwidth   \linewidth=\textwidth
 \setbox\env@box=\vbox\bgroup}%
\long\def\enddashenv{%
 \egroup
 \hsize=\hsiz@  \textwidth=\hsiz@  \linewidth=\hsiz@
 \c@breite=\d@envb   \divide\c@breite by65536
 \advance\d@envb by-\@wholewidth
 \c@hsize=\d@envb  \divide\c@hsize by65536%
 \d@envdp=\dp\env@box  \advance\d@envdp by\ht\env@box%
 \advance\d@envdp by2\fboxsep%
 \advance\d@envdp by\@wholewidth
 \d@hoehe=\d@envdp   \advance\d@hoehe by2\@wholewidth
 \c@hoehe=\d@hoehe   \divide\c@hoehe by65536
 \c@envdp=\d@envdp   \divide\c@envdp by65536%
 \c@dash=\d@dash     \divide\c@dash  by65536%
 \c@whole=\@wholewidth  \divide\c@whole by65536
 \c@half=\@halfwidth  \divide\c@half by 65536
 \noindent\unitlength 1pt
 \begin{picture}(\c@breite,\c@hoehe)(0,0)
   \put(\c@half,\c@whole){\dashbox{\c@dash}(\c@hsize,\c@envdp){\box\env@box}}
 \end{picture}%
}


\long\def\ovalenv{\@ifnextchar [{\@ovalenv}{\@ovalenv[\textwidth]}}%
\long\def\@ovalenv[#1]{%
 \hsiz@=\textwidth  \textwidth=#1  \d@envb=#1
 \advance\textwidth by-4\fboxsep
 \hsize=\textwidth   \linewidth=\textwidth
 \setbox\env@box=\vbox\bgroup}%
\long\def\endovalenv{%
 \egroup
 \hsize=\hsiz@  \textwidth=\hsiz@  \linewidth=\hsiz@
 \@wholewidth=0.4pt
 \c@breite=\d@envb   \divide\c@breite by65536
 \advance\d@envb by-2\@wholewidth
 \c@hsize=\d@envb  \divide\c@hsize by65536%
 \d@envdp=\dp\env@box  \advance\d@envdp by\ht\env@box%
 \advance\d@envdp by4\fboxsep%
 \c@envdp=\d@envdp   \divide\c@envdp by65536%
 \d@hoehe=\d@envdp   \advance\d@hoehe by2\@wholewidth
 \c@hoehe=\d@hoehe   \divide\c@hoehe by65536
 \c@tmpa=\c@hsize   \divide\c@tmpa by2%
 \c@tmpb=\c@envdp   \divide\c@tmpb by2%
 \d@tmpa=2\fboxsep   \advance\d@tmpa by\@wholewidth
 \c@xoff=\d@tmpa     \divide\c@xoff  by65536%
 \advance\d@tmpa by\dp\env@box
 \c@yoff=\d@tmpa     \divide\c@yoff  by65536%
 \unitlength 1pt\noindent
 \begin{picture}(\c@breite,\c@hoehe)(0,0)
   \put(\c@tmpa,\c@tmpb){\oval(\c@hsize,\c@envdp)}
   \put(\c@xoff,\c@yoff){\box\env@box}%
 \end{picture}%
}


==> preamble.tex <==
% *** CITATION PACKAGES ***
%
%\ifCLASSOPTIONcompsoc
  % IEEE Computer Society needs nocompress option
  % requires cite.sty v4.0 or later (November 2003)
%  \usepackage[nocompress]{cite}
%\else
  % normal IEEE
%  \usepackage{cite}
%\fi
\RequirePackage[T1]{fontenc}
\RequirePackage{graphicx}
\RequirePackage{mathptmx}      % use Times fonts if available on your TeX system
\RequirePackage{flushend}
%\RequirePackage[numbers,sort&compress]{natbib}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}

\usepackage{moreverb}

\usepackage{subfigure}

\usepackage[pdftex,svgnames,dvipsnames]{xcolor}

\usepackage{tabularx}

\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
\usepackage{algorithm}

\usepackage{url}
\usepackage{xspace}

\usepackage{amsmath}
\usepackage{amsfonts}
%\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{mathrsfs}

\usepackage{booktabs}
\usepackage{float}
\usepackage[]{microtype}

\usepackage{proof}
\usepackage{paralist}

\usepackage[]{siunitx}

\usepackage{ifthen}

\usepackage{times}
\usepackage{tablefootnote}

% \usepackage[inline,shortlabels]{enumitem}

\usepackage{fontawesome}
%\usepackage{subcaption}
\usepackage{multirow}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[pscoord]{eso-pic} % The zero point of the coordinate system is the lower left corner of the page (the default).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings}

\lstset{
    tabsize=2,
    basicstyle=\ttfamily\small,
    stringstyle=\ttfamily,
    title=\lstname,
    numbers=none,
    numberstyle=\scriptsize,
    numbersep=3pt, stepnumber=2,
    firstnumber=1,
    numberfirstline=true,
    escapeinside={(*@}{@*)},
    morekeywords={ips,ipd,pd,ps,proto,conn,url,http_access,http_reply_access,acl,allow,deny,resolution_strategy,default_action,policy_data,external_data,rule_data},
    frameround=fttt,
    aboveskip={-1\baselineskip},
}
\usepackage{array}
\usepackage{mdwmath}
\usepackage{mdwtab}

%\usepackage{fixltx2e}
\usepackage{stfloats}

\newcommand{\fw}[1]{$f\!w_{#1}$}
%\usepackage[]{units}
\usepackage{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\abovedisplayskip}{2pt}
\setlength{\belowdisplayskip}{2pt}
\setlength{\abovedisplayshortskip}{2pt}
\setlength{\belowdisplayshortskip}{2pt}
\widowpenalty10000
\clubpenalty10000



\DeclareMathOperator{\confidentiality}{\mathcal{C}}
\DeclareMathOperator{\integrity}{\mathcal{I}}
\DeclareMathOperator{\excorr}{\mathcal{E}}
\DeclareMathOperator{\Prec}{\prec}
\DeclareMathOperator{\PrecEq}{\preceq}
\DeclareMathOperator{\Succ}{\succ}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage[]{todonotes}
% \newcommand{\todoAll}[1]{\todo[color = yellow, inline]{\textbf{To all:} #1}}
% \newcommand{\todoDaniele}[1]{\todo[color = lime, inline]{\textbf{To Daniele:} #1}}
% \newcommand{\todoAldo}[1]{\todo[color = orange, inline]{\textbf{To Aldo:} #1}}
% \newcommand{\todoLeonardo}[1]{\todo[color = lime, inline]{\textbf{To Leonardo:} #1}}

%\newcommand{\complete}[1]{\textcolor{red}{COMPLETE WITH #1}}
%\newcommand{\new}[1]{{\color{blue}#1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{pdfcomment}
%\usepackage{soul}
%\newboolean{sottolinea}
%\setboolean{sottolinea}{false}
%\newboolean{risolto}
%\setboolean{risolto}{true}
%\newcommand{\sottolinea}[2]{\ifthenelse{\boolean{sottolinea}}{\pdfmarkupcomment[markup,color=yellow!30!]{#2}{#1}}{#2}}
%\newcommand{\risolto}[3]{\ifthenelse{\boolean{risolto}}{\pdfmarkupcomment[markup,color=green!30!]{#3}{(#1)\\ #2}}{#3}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cmd}[1]{\texttt{#1}\xspace}
%l2p
\newcommand{\codeRegion}[1]{c_{#1}}
\newcommand{\codeRegionSpace}{C}
\newcommand{\reducedCodeRegionSpace}{\codeRegionSpace^*}
\newcommand{\source}[1]{\operatorname{source}(\codeRegion{#1})}
\newcommand{\sLine}[1]{\operatorname{sl}(\codeRegion{#1})}
\newcommand{\eLine}[1]{\operatorname{el}(\codeRegion{#1})}
\newcommand{\protection}[1]{P_{#1}}
\newcommand{\protectionInstantiation}[1]{p_{#1}}
\newcommand{\protectionInstantiationSpace}{\mathbb{P}}
\newcommand{\protectionInstantiationSpaceLOneP}{\protectionInstantiationSpace|_{\text{AP}}}
\newcommand{\prot}[1]{\operatorname{protection}(\protectionInstantiation{#1})}
\newcommand{\appliedProtectionInstantiation}[2]{\protectionInstantiation{#1}/\codeRegion{#2}}
\newcommand{\biSet}{\{ 0, 1 \}}
\newcommand{\overh}[1]{\operatorname{\mathscr{O}}_{#1}}
\newcommand{\overhead}[3]{\overh{#1}(\appliedProtectionInstantiation{#2}{#3})}
\newcommand{\overheadd}[4]{\overh{#1}(\appliedProtectionInstantiation{#2}{#3}, \metric{1}{#3}, \metric{2}{#3}, \dots)}
\newcommand{\localOverhead}[3]{\operatorname{\omega}_{#1}(\appliedProtectionInstantiation{#2}{#3})}
\newcommand{\metric}[2]{\operatorname{\mathcal{M}}_{#1}(\codeRegion{#2})}
\newcommand{\protectionInstantiationSpaceMax}{\Gamma}
\newcommand{\overheadMax}[1]{\Omega_{#1}}
\newcommand{\techniques}{\mathbb{T}}
\newcommand{\replication}{\mathcal{R}}
\newcommand{\enlargement}{\mathcal{E}}
\newcommand{\shadowing}{\mathcal{S}}
\newcommand{\confusion}[3]{\operatorname{cnf}_{#1}(\appliedProtectionInstantiation{#2}{#3})}
\newcommand{\confusionLong}[3]{\operatorname{cnf}_{#1,\protectionInstantiation{#2}}(#3)}
\newcommand{\confusionShadowing}[3]{\operatorname{cnf}_{\shadowing}(\appliedProtectionInstantiation{#1}{#3},\appliedProtectionInstantiation{#2}{#3})}
\newcommand{\confusionShadowingLong}[3]{\operatorname{cnf}_{\shadowing,\protectionInstantiation{#1},\protectionInstantiation{#2}}(#3)}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\lOneP}[2]{\operatorname{AP}(\appliedProtectionInstantiation{#1}{#2})}
\newcommand{\rLOneP}[2]{\operatorname{AP^*}(\appliedProtectionInstantiation{#1}{#2})}
\newcommand{\prox}[2]{\operatorname{adj}(\codeRegion{#1}, \codeRegion{#2})}
\newcommand{\mainVariable}[2]{x_{\appliedProtectionInstantiation{#1}{#2}}}
\newcommand{\orderVariable}[3]{y_{\codeRegion{#1}, \protectionInstantiation{#2}, \protectionInstantiation{#3}}}
\newcommand{\proxVariable}[3]{g_{\codeRegion{#1}, \codeRegion{#2}, \protectionInstantiation{#3}}}
\newcommand{\proxSet}[3]{G_{\codeRegion{#1}, \codeRegion{#2}, \protectionInstantiation{#3}}}
\newcommand{\enlargementVariable}[3]{e_{\codeRegion{#1}, \codeRegion{#2}, \protectionInstantiation{#3}}}
\newcommand{\enlargementSet}[2]{E_{\appliedProtectionInstantiation{#1}{#2}}}
\newcommand{\techniqueVariable}[2]{z_{\appliedProtectionInstantiation{#1}{#2}}}
\newcommand{\parent}[1]{\operatorname{parent}(\codeRegion{#1})}
\newcommand{\children}[1]{\operatorname{children}(\codeRegion{#1})}
\newcommand{\ancestors}[1]{\operatorname{ancestors}(\codeRegion{#1})}
\newcommand{\descendants}[1]{\operatorname{descendants}(\codeRegion{#1})}
%\newcommand{\weight}[1]{\operatorname{weight}(\codeRegion{#1})}
\newcommand{\bonus}[3]{\rho^{#1}_{\appliedProtectionInstantiation{#2}{#3}}}
\newcommand{\orderSet}[2]{\Psi_{\appliedProtectionInstantiation{#1}{#2}}}
\newcommand{\LUP}{asset protection\xspace}
\newcommand{\LDP}{asset hiding\xspace}
\newcommand{\High}{\textsc{high}\xspace}
\newcommand{\Low}{\textsc{low}\xspace}
\newcommand{\None}{\textsc{--}}
\newcommand{\Masking}[2]{#1 (#2)}

%latex stuff
\newcommand{\Center}[1]{\multicolumn{1}{c}{#1}}
\newcommand{\header}[2]{\multicolumn{#1}{c}{\textsc{#2}}}

\usepackage[acronym,nomain]{glossaries}
%\makeglossaries
\glsdisablehyper
%metamodel compatibility
\newcommand{\class}[1]{{\footnotesize\sffamily#1}}
\newcommand{\association}[1]{{\footnotesize\sffamily#1}}
\let\attribute\attr
\newcommand{\attribute}[1]{{\footnotesize\sffamily#1}}
%\newcommand{\changed}[1]{#1}
\newcommand{\changed}[1]{{\color{black}#1}}
\definecolor{mypinka}{rgb}{0.858, 0.188, 0.478}
\definecolor{mypinkb}{rgb}{0.708, 0.438, 0.528}
\newcommand{\changeda}[1]{{\color{mypinka}#1}}
\newcommand{\changedb}[1]{{\color{mypinkb}#1}}

% Abbreviations.
\newcommand{\ie}{i.e.,\@\xspace} % Id est.
\newcommand{\eg}{e.g.,\@\xspace} % Exempli gratia.
\newcommand{\wrt}{w.r.t.\@\xspace} % With respect to.
\newcommand{\etal}{\textit{~et~al.\@}\xspace}

\newcommand{\ekb}{Knowledge Base\xspace}
\newcommand{\esca}{Source Code Analyzer\xspace}
\newcommand{\emf}{Metrics Framework\xspace}
\newcommand{\eptc}{Protection Tools Connector\xspace}
%\newacronym{ear}{EAR}{\gls{ear} Attack Reasoner}\newcommand{\ear}{\gls{ear}\xspace}
\newcommand{\ebad}{Risk Assessment Engine\xspace}
\newcommand{\eape}{Protection Enumerator\xspace}
\newcommand{\eapd}{Risk Mitigation Engine\xspace}
\newcommand{\ehal}{Asset Hiding Engine\xspace}
\newcommand{\esd}{Solution Deployer\xspace}
\newcommand{\eui}{User Interface\xspace}


\newacronym{dsr}{DSR}{Design-Science Research}\newcommand{\dsr}{\gls{dsr}\xspace}
\newacronym{feds}{FEDS}{Framework For Evaluation of Design Science}\newcommand{\feds}{\gls{feds}\xspace}

%ESP data (pis, ecc.)
\newacronym{as}{AS}{Attack Step}\newcommand{\AS}{\gls{as}\xspace}
\newcommand{\ASs}{\glspl{as}\xspace}
\newacronym{ap}{AP}{Attack Path}
\newcommand{\AP}{\gls{ap}\xspace}
\newcommand{\APs}{\glspl{ap}\xspace}
\newacronym{dpi}{DPI}{Deployed Protection Instance}\newcommand{\DPI}{\gls{dpi}\xspace}
\newcommand{\DPIs}{\glspl{dpi}\xspace}
\newcommand{\DPIset}{\DPI set\xspace}
\newcommand{\DPIsets}{\DPI sets\xspace}
\newacronym{pi}{PI}{Protection Instance}
\newcommand{\PI}{\gls{pi}\xspace}
\newcommand{\PIs}{\glspl{pi}\xspace}
\newcommand{\PIset}{\PI set\xspace}
\newcommand{\PIsets}{\PI sets\xspace}
\newacronym{po}{PO}{{Protection Objective}}\newcommand{\PO}{\gls{po}\xspace}
\newcommand{\POs}{\glspl{po}\xspace}
\newcommand{\POset}{\gls{po} set\xspace}
\newcommand{\POsets}{\glspl{po} sets\xspace}
%\newacronym{cr}{CR}{Code Region}\newcommand{\CR}{\gls{cr}\xspace}
%	\newcommand{\CRs}{\glspl{cr}\xspace}
\newcommand{\CR}{code region\xspace}
\newcommand{\CRs}{code regions\xspace}
\newcommand{\CRset}{\CR set\xspace}
\newcommand{\CRsets}{\CR sets\xspace}
%institutions
\newacronym{nist}{NIST}{National Institute of Standards and Technology}\newcommand{\nist}{\gls{nist}\xspace}
\newacronym{gdpr}{GDPR}{General Data Protection Regulation}\newcommand{\gdpr}{\gls{gdpr}\xspace}

%aspire miscellanea
\newacronym{asp}{ASPIRE}{Advanced Software Protection: Integration, Research and Exploitation}\newcommand{\asp}{\gls{asp}\xspace}
\newacronym{accl}{ACCL}{Client-side Communication Logic}\newcommand{\accl}{\gls{accl}\xspace}
\newacronym{ascl}{ASCL}{Server-side Communication Logic}\newcommand{\ascl}{\gls{ascl}\xspace}
\newacronym{actc}{ACTC}{ASPIRE Compiler Tool Chain}\newcommand{\actc}{\gls{actc}\xspace}
\newacronym{esp}{ESP}{Expert system for Software Protection}\newcommand{\esp}{\gls{esp}\xspace}
\newacronym{it}{IT}{Information Technology}\newcommand{\itech}{\gls{it}\xspace}


%software protection acronyms
\newacronym{diablo}{DIABLO}{Diablo Is A Better Link-time Optimizer}\newcommand{\diablo}{\gls{diablo}\xspace}
\newacronym{cff}{CFF}{Control Flow Flattening}\newcommand{\cff}{\gls{cff}\xspace}
\newacronym{api}{API}{Application Programming Interface}\newcommand{\api}{\gls{api}\xspace}
\newacronym{ip}{IP}{Intellectual Property}\newcommand{\ip}{\gls{ip}\xspace}
\newacronym{drm}{DRM}{Digital Rights Management}\newcommand{\drm}{\gls{drm}\xspace}
\newacronym{cve}{CVE}{Common Vulnerabilities and Exposures}\newcommand{\cve}{\gls{cve}\xspace}
\newacronym{cwe}{CWE}{Common Weakness Enumeration}\newcommand{\cwe}{\gls{cwe}\xspace}
\newacronym{mate}{MATE}{Man-At-The-End}\newcommand{\mate}{\gls{mate}\xspace}
\newacronym{sp}{SP}{Software Protection}\newcommand{\softprot}{\gls{sp}\xspace}
\newacronym{aslr}{ASLR}{Address Space Layout Randomization}\newcommand{\aslr}{\gls{aslr}\xspace}
%attestation acronyms
\newacronym{txt}{TXT}{Trusted eXecution Technology}\newcommand{\txt}{\gls{txt}\xspace}
\newacronym{tpm}{TPM}{Trusted Platform Module}\newcommand{\tpm}{\gls{tpm}\xspace}
\newacronym{tcg}{TCG}{Trusted Computing Group}\newcommand{\tcg}{\gls{tcg}\xspace}
\newacronym{sgx}{SGX}{Software Guard Extensions}\newcommand{\sgx}{\gls{sgx}\xspace}

%for old times sake
\newacronym{dec}{DEC}{Digital Equipment Corporation}\newcommand{\dec}{\gls{dec}\xspace}
\newacronym{vax}{VAX}{Virtual Address eXtension}\newcommand{\vax}{\gls{vax}\xspace}

%expert systems
\newacronym{dendral}{DENDRAL}{DENDritic ALgorithm}\newcommand{\dendral}{\gls{dendral}\xspace}
\newacronym{xcon}{XCON}{eXpert CONfigurer}\newcommand{\xcon}{\gls{xcon}\xspace}
\newacronym{ides}{IDES}{Intrusion Detection Expert System}\newcommand{\ides}{\gls{ides}\xspace}
\newacronym{nides}{NIDES}{Next-generation Intrusion Detection Expert System}\newcommand{\nides}{\gls{nides}\xspace}
\newacronym{nidx}{NIDX}{Network Intrusion Detection eXpert system}\newcommand{\nidx}{\gls{nidx}\xspace}
\newacronym{nadir}{NADIR}{Network Anomaly Detection and Intrusion Reporter}\newcommand{\nadir}{\gls{nadir}\xspace}
\newacronym{audes}{AudES}{Expert System for security Auditing}\newcommand{\audes}{\gls{audes}\xspace}

%software acronyms
\newacronym{cfg}{CFG}{Control Flow Graph}\newcommand{\cfg}{\gls{cfg}\xspace}
\newacronym{os}{OS}{Operating System}\newcommand{\os}{\gls{os}\xspace}
\newacronym{dll}{DLL}{Dynamic-Link Library}\newcommand{\dll}{\gls{dll}\xspace}
\newacronym{gnu}{GNU}{GNU is Not Unix}\newcommand{\gnu}{\gls{gnu}\xspace}
\newacronym{gcc}{GCC}{\gls{gnu} C Compiler}\newcommand{\gcc}{\gls{gcc}\xspace}
\newacronym{gdb}{GDB}{\gls{gnu} DeBugger}\newcommand{\gdb}{\gls{gdb}\xspace}
\newacronym{foss}{FOSS}{Free and Open Source Software}\newcommand{\foss}{\gls{foss}\xspace}
\newacronym{cdt}{CDT}{C/C++ Development Tooling}\newcommand{\cdt}{\gls{cdt}\xspace}
\newacronym{ast}{AST}{Abstract Syntax Tree}\newcommand{\astree}{\gls{ast}\xspace}
\newacronym{gui}{GUI}{Graphical User Interface}\newcommand{\gui}{\gls{gui}\xspace}
\newacronym{xml}{XML}{eXtensible Mark-up Language}\newcommand{\xml}{\gls{xml}\xspace}

%metrics acronyms
\newacronym{sloc}{SLOC}{Source Lines Of Code}\newcommand{\sloc}{\gls{sloc}\xspace}
\newacronym{hl}{HL}{Halstead's Length}\newcommand{\HL}{\gls{hl}\xspace}
\newacronym{cc}{CC}{Cyclomatic Complexity}\newcommand{\CC}{\gls{cc}\xspace}

%hardware acronyms
\newacronym{cpu}{CPU}{Central Processing Unit}\newcommand{\cpu}{\gls{cpu}\xspace}
\newacronym{fpu}{FPU}{Floating Point Unit}\newcommand{\fpu}{\gls{fpu}\xspace}
\newacronym{alu}{ALU}{Arithmetic and Logic Unit}\newcommand{\alu}{\gls{alu}\xspace}
\newacronym{gpu}{GPU}{Graphics Processing Unit}\newcommand{\gpu}{\gls{gpu}\xspace}
\newacronym{gpgpu}{GPGPU}{General-Purpose computing on Graphics Processing Units}\newcommand{\gpgpu}{\gls{gpgpu}\xspace}


%programming languages acronyms
\newacronym{lisp}{LISP}{LISt Processor}\newcommand{\lisp}{\gls{lisp}\xspace}
\newacronym{cil}{CIL}{C Intermediate Language}\newcommand{\cil}{\gls{cil}\xspace}

%network acromyms
\newacronym{smb}{SMB}{Server Message Block}\newcommand{\smb}{\gls{smb}\xspace}

%network protection acronyms
\newacronym{mitm}{MITM}{Man-In-The-Middle}\newcommand{\mitm}{\gls{mitm}\xspace}
\newacronym{ddos}{DDoS}{Distributed Denial of Service}\newcommand{\ddos}{\gls{ddos}\xspace}

%malware acronyms
\newacronym{rat}{RAT}{Remote Access Trojan}\newcommand{\rat}{\gls{rat}\xspace}

%network protection
\newacronym{ids}{IDS}{Intrusion Detection System}\newcommand{\ids}{\gls{ids}\xspace}
\newacronym{cysemol}{CySeMoL}{Cyber Security Modeling Language}\newcommand{\cysemol}{\gls{cysemol}\xspace}
\newacronym{camel}{CAMEL}{Cloud Application Modelling \& Execution Language}\newcommand{\camel}{\gls{camel}\xspace}
%machine learning
\newacronym{ml}{ML}{Machine Learning}\newcommand{\ml}{\gls{ml}\xspace}
\newacronym{ai}{AI}{Artificial Intelligence}\newcommand{\ai}{\gls{ai}\xspace}
\newacronym{som}{SOM}{Self-Organizing Maps}\newcommand{\som}{\gls{som}\xspace}
\newacronym{ann}{ANN}{Artificial Neural Network}\newcommand{\ann}{\gls{ann}\xspace}

%optimization
\newacronym{milp}{MILP}{Mixed Integer-Linear Programming}\newcommand{\milp}{\gls{milp}\xspace}

%ontologies
\newacronym{owl}{OWL}{Web Ontology Language}\newcommand{\owl}{\gls{owl}\xspace}
\newacronym{owltwo}{OWL2}{\acrlong{owl} 2}\newcommand{\owltwo}{\gls{owltwo}\xspace}

%other stuff
\newacronym{roi}{ROI}{Return In Investment}\newcommand{\roi}{\gls{roi}\xspace}
\newacronym{byod}{BYOD}{Bring Your Own Device}\newcommand{\byod}{\gls{byod}\xspace}
\newacronym{bsa}{BSA}{BSA | The Software Alliance}\newcommand{\bsa}{\gls{bsa}\xspace}
\newacronym{otp}{OTP}{One-Time Password}\newcommand{\otp}{\gls{otp}\xspace}
\newacronym{pin}{PIN}{Personal Identification Number}\newcommand{\pin}{\gls{pin}\xspace}
\newacronym{sdlc}{SDLC}{Software Development Life Cycle}\newcommand{\sdlc}{\gls{sdlc}\xspace}
\newacronym{kb}{KB}{Knowledge Base}\newcommand{\kb}{\gls{kb}\xspace}
\newacronym{poc}{PoC}{Proof of Concept}\newcommand{\poc}{\gls{poc}\xspace}
\newacronym{sto}{StO}{Security-through-Obscurity}\newcommand{\sto}{\gls{sto}\xspace}

\usepackage{tikz}
\usetikzlibrary{
	decorations,
	arrows,
	shapes,positioning,
	patterns,
	fit,
	automata,
	decorations.markings,
	plotmarks,
	decorations.pathmorphing,
	positioning,
	backgrounds,
	fit,
	calc,
	arrows.meta}

\usepackage{pgfplots}
\pgfplotsset{ cycle list={%
		{smooth,black,mark=triangle*},
		{smooth,black,mark=triangle},
		{smooth,black,mark=*},
		{smooth,black,mark=o},
		{smooth,black,mark=square*},
		{smooth,black,mark=square},
		{smooth,black,mark=diamond*},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
	},
	compat=1.3,
	tick label style={ font=\scriptsize,/pgf/number format/set thousands separator={}}}
\usepgfplotslibrary{fillbetween}


\usepackage[draft]{fixme}
\fxsetup{layout=inline,theme=color}
\FXRegisterAuthor{bds}{brds}{\color{purple}bds}
\FXRegisterAuthor{ab}{aab}{\color{brown}ab}
\FXRegisterAuthor{bc}{ebc}{\color{red}bc}
\FXRegisterAuthor{lr}{alr}{\color{orange}lr}
\FXRegisterAuthor{dc}{adc}{\color{green!50!black}dc}

\FXRegisterAuthor{rone}{roner}{\color{pink}reviewer1}
\FXRegisterAuthor{rtwo}{rtwor}{\color{pink}reviewer2}
\FXRegisterAuthor{rthree}{rthreer}{\color{pink}reviewer3}

%%%%%%%%%%%%%%%%%%%%5
% for arxiv only
%\usepackage[pscoord]{eso-pic}
\newcommand{\placetextbox}[3]{% \placetextbox{<horizontal pos>}{<vertical pos>}{<stuff>}
 \setbox0=\hbox{#3}% Put <stuff> in a box
 \AddToShipoutPictureFG*{% Add <stuff> to current page foreground
    \put(\LenToUnit{#1\paperwidth},\LenToUnit{#2\paperheight}){\vtop{{\null}\makebox[0pt][c]{#3}}}%
 }%
}%

\usepackage[normalem]{ulem}
%\usepackage{xpatch}
%\xpatchcmd{\dashuline}
%  {\bgroup}
%  {\bgroup\def\ULthickness{2pt}}
%  {}{}

\usepackage[dvipsnames]{xcolor}

\newcounter{bubbles}
\setcounter{bubbles}{1}
\newcounter{bubbless}
\setcounter{bubbless}{1}
\newcounter{bubblesf}
\setcounter{bubblesf}{1}
\newcounter{bubblesr}
\setcounter{bubblesr}{1}
\newcounter{bubbleso}
\setcounter{bubbleso}{1}
\newcounter{bubblesrd}
\setcounter{bubblesrd}{1}
\newcounter{bubblesa}
\setcounter{bubblesa}{1}
\newcounter{bubblesc}
\setcounter{bubblesc}{1}
\newcounter{bubblesm}
\setcounter{bubblesm}{1}
\newcounter{bubblesM}
\setcounter{bubblesM}{1}

\newcommand*\encircle[2]{  \tikz[baseline=(char.base)] 
    \node[draw=#2!90!black, shape=circle, inner sep=1pt, fill=#2,  text=white,line width=1pt] (char) { #1};}

\newcommand*\encircled[2]{  \tikz[baseline=(char.base)] 
    \node[draw=#2!90!black, shape=rectangle, inner sep=1pt, fill=#2,  text=white,line width=1pt] (char) { #1};}


\newcommand{\construct}[1]{\hyperdef{construct}{\arabic{bubblesc}}{{\color{black}\encircled{\scriptsize c.\arabic{bubblesc}\stepcounter{bubblesc}}{black}~\dashuline{\hspace*{-1pt}~#1}}}}
\newcommand{\constructlab}[1]{\hyperlink{construct.#1}{\encircled{\scriptsize c.#1}{black}}}

\newcommand{\introconstruct}[1]{{\color{black}\encircled{\scriptsize c.X}{black}~\dashuline{\hspace*{-1pt}~#1}}}


\newcommand{\model}[1]{\hyperdef{model}{\arabic{bubblesM}}{{\color{black}\encircled{\scriptsize M.\arabic{bubblesM}\stepcounter{bubblesM}}{Gray}~\dashuline{\hspace*{-1pt}~#1}}}}
\newcommand{\modellab}[1]{\hyperlink{model.#1}{\encircled{\scriptsize M.#1}{Gray}}}

\newcommand{\intromodel}[1]{{\color{black}\encircled{\scriptsize M.X}{Gray}~\dashuline{\hspace*{-1pt}~#1}}}

\newcommand{\method}[1]{\hyperdef{method}{\arabic{bubblesm}}{{\color{black}\encircled{\scriptsize m.\arabic{bubblesm}\stepcounter{bubblesm}}{Purple}~\dashuline{\hspace*{-1pt}~#1}}}}
\newcommand{\methodlab}[1]{\hyperlink{method.#1}{\encircled{\scriptsize m.#1}{Purple}}}

\newcommand{\intromethod}[1]{{\color{black}\encircled{\scriptsize m.X}{Purple}~\dashuline{\hspace*{-1pt}~#1}}}

\newcommand{\concept}[1]{{\color{black}\encircled{\scriptsize c.\arabic{bubbles}\stepcounter{bubbles}}{black}~\dashuline{\hspace*{-1pt}~#1}}}

\newcommand{\conceptlab}[1]{\encircled{\scriptsize c.#1}{black}}

\newcommand{\introconcept}[1]{{\color{black}\encircled{\scriptsize c.X}{black}~\dashuline{\hspace*{-1pt}~#1}}}

\newcommand{\introsota}[1]{{\color{black}\encircled{\scriptsize s.X}{RedOrange}\dashuline{\hspace*{-1pt}~#1}}}

\newcommand{\sota}[1]{{\color{black}\encircled{\scriptsize s.\arabic{bubbless}\stepcounter{bubbless}}{RedOrange}\dashuline{\hspace*{-1pt}~#1}}}

\newcommand{\sotalab}[1]{{\encircled{\scriptsize s.#1}{RedOrange}}}

\newcommand{\futurework}[1]{\hyperdef{futurework}{\arabic{bubblesf}}{{\color{black}\encircled{{\scriptsize f.\arabic{bubblesf}\stepcounter{bubblesf}}}{RoyalBlue}\dashuline{\hspace*{-1pt}~#1}}}}

\newcommand{\futureworklab}[1]{\hyperlink{futurework.#1}{\encircled{\scriptsize f.#1}{RoyalBlue}}}


\newcommand{\introfuturework}[1]{{\color{black}\encircled{{\scriptsize f.X}}{RoyalBlue}\dashuline{\hspace*{-1pt}~#1}}}

\newcommand{\recommendation}[1]{{\color{black}\encircled{\scriptsize r.\arabic{bubblesr}\stepcounter{bubblesr}}{PineGreen}\dashuline{\hspace*{-1pt}~#1}}}
\newcommand{\recommendationlab}[1]{{\encircled{\scriptsize r.#1}{PineGreen}}}


\newcommand{\introrecommendation}[1]{{\color{black}\encircled{\scriptsize r.X}{PineGreen}\dashuline{\hspace*{-1pt}~#1}}}

%\newcommand{\recopen}[1]{\color{black}\encircle{r}{teal}\color{black}\encircle{{\small ?}}{Cerulean}\dashuline{\hspace*{-2pt}~#1}}

\newcommand{\openissue}[1]{\hyperdef{openissue}{\arabic{bubbleso}}{{\color{black}\encircled{{\scriptsize ?.\arabic{bubbleso}\stepcounter{bubbleso}}}{CornflowerBlue}\dashuline{\hspace*{-1pt}~#1}}}}
\newcommand{\openissuelab}[1]{\hyperlink{openissue.#1}{\encircled{\scriptsize ?.#1}{CornflowerBlue}}}


\newcommand{\introopenissue}[1]{{\color{black}\encircled{{\scriptsize ?.X}}{CornflowerBlue}\dashuline{\hspace*{-1pt}~#1}}}



\newcommand{\researchdir}[1]{\hyperdef{researchdir}{\arabic{bubblesrd}}{{\color{black}\encircled{{\scriptsize !.\arabic{bubblesrd}\stepcounter{bubblesrd}}}{Mahogany}\dashuline{\hspace*{-1pt}~#1}}}}
\newcommand{\introresearchdir}[1]{{\color{black}\encircled{{\scriptsize !.X}}{Mahogany}\dashuline{\hspace*{-1pt}~#1}}}
\newcommand{\researchdirlab}[1]{\hyperlink{researchdir.#1}{\encircled{\scriptsize !.#1}{Mahogany}}}



\newcommand{\automationreq}[1]{{\color{black}\encircled{\scriptsize a.\arabic{bubblesa}\stepcounter{bubblesa}}{orange}\dashuline{\hspace*{-1pt}~#1}}}
\newcommand{\automationreqlab}[1]{{\encircled{\scriptsize a.#1}{orange}}}

\newcommand{\introautomationreq}[1]{{\color{black}\encircled{\scriptsize a.X}{orange}\dashuline{\hspace*{-1pt}~#1}}}
%\newcommand{\git}[1]{{\color{black}\encircle{a}{YellowOrange}\dashuline{\hspace*{-2pt}~#1}}}

% \newcomand{\sota}{\scalerel*{\includegraphics{images/bricks.png}}{b} #1}
%\newcommand{\sota}[1]{{\color{black}\wave{\textdollar~#1}}}
%\newcommand{\futurework}[1]{{\color{black}\dashuline{$\mathcal{F}$~#1}}}
%\newcommand{\recommendation}[1]{{\color{black}\dashuline{\textregistered~#1}}}
%\newcommand{\openissue}[1]{{\color{black}\dashuline{$\mathcal{O}$~#1}}}
%\newcommand{\researchdir}[1]{{\color{black}\dashuline{$\mathcal{D}$~#1}}}
%\newcommand{\automationreq}[1]{{\color{black}\dashuline{$\mathcal{A}$~#1}}}


\usepackage{booktabs}

\input{pkgpicins}
\input{pkgnumcompress}

\urlstyle{same}


% \usepackage{mdframed}
% \mdfdefinestyle{paper_frame}{%
%     linecolor=black,
%     outerlinewidth=1pt,
%     roundcorner=20pt,
%     innertopmargin=4pt,
%     innerbottommargin=4pt,
%     innerrightmargin=4pt,
%     innerleftmargin=4pt,
%         leftmargin = 4pt,
%         rightmargin = 4pt
%     backgroundcolor=gray!50!white}

\usepackage{tcolorbox}
\tcbuselibrary{breakable}
